Accelerated Reinforcement Learning for Temporal Logic Control Objectives

This paper addresses the problem of learning control policies for mobile robots, modeled as unknown Markov Decision Processes (MDPs), that are tasked with temporal logic missions, such as sequencing, coverage, or surveillance. The MDP captures uncertainty in the workspace structure and the outcomes of control decisions. The control objective is to synthesize a control policy that maximizes the probability of accomplishing a high-level task, specified as a Linear Temporal Logic (LTL) formula. To address this problem, we propose a novel accelerated model-based reinforcement learning (RL) algorithm for LTL control objectives that is capable of learning control policies significantly faster than related approaches. Its sample-efficiency relies on biasing exploration towards directions that may contribute to task satisfaction. This is accomplished by leveraging an automaton representation of the LTL task as well as a continuously learned MDP model. Finally, we provide comparative experiments that demonstrate the sample efficiency of the proposed method against recent RL methods for LTL objectives.

==> algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> files/alg.tex <==
%ASSUMPTIONS

%Disjoint regions? no reachable regions? not in the PF but possibly needed to ensure completeness separable regions? only for completeness



%\subsection{Planning for Information Acquisition}
To solve Problem \ref{prob}, we propose a novel distributed reactive planning algorithm that designs on-the-fly new local paths as new obstacles are discovered. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 
%

\begin{algorithm}[t]
%\footnotesize
\caption{Reactive LTL Planning in Unknown Environments}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) initial robot configuration $\bbp(0)$, (ii) LTL formula $\phi$}
\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
Convert $\phi$ into a DFA\label{rrt:dfa}\;
%Initial state $\bbq(0)=[\bbp(0), q_D^0]$;\label{rrt:init}
Initialize $t=0$\;\label{rrt:t0}
%Update current DFA state as $q_D(0)=\delta(q_D^0,L(\bbp(0)))$\;
Prune DFA\;\label{rrt:prune}
Select an initial state $q_D(0)=q_D^0$ and a feasible final state $q_F^{\text{feas}}$\;\label{rrt:feasFinal}
%Current DFA state $q_D(t)=q_D^0$\;\label{rrt:init}
%Compute distance from $q_D(t)$ to $q_D^F$\;
\If{$\nexists q_D^0, q_F$ such that $d(q_D^0, q_F)\neq \infty$}{
Error message: \textit{$\phi$ cannot be satisfied}\;}\label{eq:unsat}
Select a DFA target state $q_D^{\text{target}}$\;\label{rrt:selTarget}
Initialize $\texttt{updateLoc}=0$ and $\texttt{updateDFA}=0$\;
\While{$q_D(t)\notin \ccalQ_F$}{
%
\If{$(q_D(t)=q_D^{\text{target}})\vee (\texttt{updateDFA}=1)$}{
Select a new DFA target state $q_D^{\text{target}}$\;\label{rrt:updTarget}
%
Collect in the set $\ccalL$ the locations/regions that enable a transition from $q_D(t)$ to $q_D^{\text{target}}$\;
%
Select a location/regions $\bbq^{\text{target}}$ among those in $\ccalL$\;
$\texttt{updateDFA}=0$\;
}
%
\If{$\texttt{updateLoc}=1$}{
Select a new location/region $\bbq^{\text{target}}$ from $\ccalL$\;
$\texttt{updateLoc}=0$\;
}
%
Temporary set of obstacles $\hat{O}$ collects known obstacles and regions (excluding those in $\ccalL$) that enable transitions to DFA states $q_D$ that satisfy $q_D\neq q_D(t)$ and $q_D\neq q_D^{\text{target}}$\;
%
\If{$\bbq^{\text{target}}$ reachable}{
Apply a control input $\bbu$ that decreases the geodesic distance (using $\hat{O}$) between $\bbp(t)$ and the desired location $\bbq^{\text{target}}$: $\bbp(t+1)=f(\bbp(t),\bbu)$\;
%
Update current DFA state $q_D(t+1)$ based on current observation $L(\bbp(t+1))$\;}
%
\Else{
Update the set $\ccalL$: $\ccalL=\ccalL\setminus\{\bbq^{\text{target}}\}$\;
\texttt{updateLoc}=1\;
\If{$\ccalL=\emptyset$}{
Update pruning of DFA\;
\texttt{updateDFA}=1\;
}
}
%
Update current map by incorporating sensor measurements\;
%
$t=t+1$\;
}
Among all nodes in $\ccalX_g$, find $\bbq_{\text{end}}(t_{\text{end}})$ \; \label{rrt:node}
$H=t_{\text{end}}$ and recover $\bbu_{0:H}$ by computing the path $\bbq_{0:t_{\text{end}}}= \bbq(0), \dots, \bbq(t_{\text{end}}) $\;\label{rrt:solution}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize


First, we translate the specification $\phi$ constructed using a set of atomic predicates $\mathcal{AP}$ into Deterministic Finite state Automaton (DFA), defined as follows \cite{baier2008principles} [line \ref{rrt:dfa}, Alg. \ref{alg:RRT}]. %Given a temporal logic formula $\phi$ , with syntax and semantics as described in Definitions \ref{syntax} and \ref{semantics}, respectively, a DFA is defined as follows:

\begin{definition}[DFA]
A Deterministic Finite state Automaton (DFA) $D$ over $2^{\mathcal{AP}}$ is defined as a tuple $D=\left(\ccalQ_{D}, \ccalQ_{D}^0,\rightarrow_D,\mathcal{Q}_F\right)$, where $\ccalQ_{D}$ is the set of states, $\ccalQ_{D}^0\subseteq\ccalQ_{D}$ is a set of initial states, $\rightarrow_{D}\subseteq\ccalQ_{D}\times 2^{\mathcal{AP}}\times\ccalQ_{D}$ is the transition relation, and $\ccalQ_F\subseteq\ccalQ_{D}$ is a set of accepting/final states. 
\end{definition}
A run of $\rho_D$ of $D$ over a finite word $\sigma\in(2^{\mathcal{AP}})^*$, is a sequence $\rho_D=q_D^0q_D^1q_D^2\dots,q_D^K$, where $q_D^0\in\ccalQ_D^0$ and $(q_D^{k},\sigma(k+1),q_D^{k+1})\in\rightarrow_{D}$, $\forall k\in\mathbb{N}$. A run $\rho_D$ is called \textit{accepting} if there exists $k\in\{0,\dots,K\}$, such that $q_k\in\ccalQ_F$. %The words $\sigma$ that result in an accepting run of $D$ constitute the accepted language of $D$.

The proposed distributed algorithm builds paths that live in the infinite-dimensional space $\Omega^N\times\ccalQ_D$ online. The synthesized paths are updated as the map of the environment is updated. In what follows, we denote by $q_D(t)$ the DFA state of the multi-robot system at time $t$. We initialize $q_D(0)$ as $q_D(0)=q_D^0$, for some $q_D^0\in\ccalQ_D^0$ [line \ref{rrt:feasFinal}, Alg. \ref{alg:RRT}]. The main idea of Algorithm \ref{alg:RRT} is that at any time $t$, given the state $q_D(t)$ the robots collaboratively select a target DFA state, denoted by $q_D^{\text{target}}$ that is (i) reachable from $q_D(t)$, and (ii) `closer' to the set of final states $\ccalQ_F$ according to a distance metric defined over the DFA; see Section \ref{sec:prune}. Given the state $q_D^{\text{target}}$, the robots move towards locations that will enable the transition from $q_D(t)$ to $q_D^{\text{target}}$ while updating the current map and avoiding previously unforeseen obstacles. Once this transition is enabled, the robots update the target DFA state $q_D^{\text{target}}$ until they reach a final DFA state.%\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%

%By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, while the cost of a node $\bbq(t+1)=[\bbp(t+1), q_D]\in\ccalV$, given its parent node $\bbq(t)=[\bbp(t),q_D']\in\ccalV$, is computed as 
%\begin{equation}\label{eq:costUpd}
%J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  w(\bbp(t),\bbp(t+1)).
%\end{equation}
%Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.

 


\subsection{Pruning the DFA}\label{sec:prune}
Given the DFA $D$, the next step is to prune it by removing transitions that cannot be enabled [line \ref{rrt:prune}, Alg. \ref{alg:RRT}]. This is required to define a distance function over the state-space of the DFA. %
%
Specifically, the pruned DFA is constructed by removing all infeasible DFA transitions. A \textit{feasible} DFA transition is defined as follows.

%To define the feasible DFA transitions we need first to introduce the following definitions. Let $b_{\text{inv}}^{q_D}$ denote the Boolean formula that if satisfied by $\sigma_{\text{inv}}\in\Sigma$, then $q_D=\delta(q_D,\sigma_{\text{inv}})$. Let also $b_{\text{next}}^{q_D,q_D'}$ denote the Boolean formula that if satisfied by $\sigma_{\text{next}}\in\Sigma$, then $q_D'=\delta(q_D,\sigma_{\text{next}})$. 
%
%We also rewrite $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$ as follows:
%\begin{equation}\label{eq:eq1}
%    b_{\text{inv}}^{q_D} = b_{\text{inv}}^{\text{goal}} \triangle (\neg b_{\text{inv}}^{\text{avoid}} ),
%\end{equation}

%\begin{equation}\label{eq:eq2}
%    b_{\text{next}}^{q_D,q_D'} = b_{\text{next}}^{\text{goal}} \triangle (\neg b_{\text{next}}^{\text{avoid}} ),
%\end{equation}
%where in the Boolean formulas  $b_{\text{next}}^{\text{goal}}$, $b_{\text{next}}^{\text{avoid}}$, $b_{\text{inv}}^{\text{goal}}$ and $b_{\text{inv}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:eq1} and \eqref{eq:eq2}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator.

We also need to define when a word $\sigma\in\Sigma$ is \textit{feasible}, i.e., when it can be generated by the multi-robot system. To this end, we first need to define the words $\sigma_j\in\Sigma_j=2^{\mathcal{AP}_j}$ that are feasible, i.e, the words that can be generated by robot $j$ \cite{kantaros2018text}. % defined in \ref{defn:wTS}.%\footnote{Recall from Definition \ref{defn:wTS} that $\text{wTS}_i$ is defined over $\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma_i=2^{\mathcal{AP}_i}$. Also, recall from Definition \ref{def:pts} that the PTS is defined over $\mathcal{AP}=\bigcup_{i=1}^N\mathcal{AP}_i$ and, therefore, its alphabet is $\Sigma=2^{\mathcal{AP}}$. Also, throughout the paper, we denote the finite words by $\sigma^*\in\Sigma$ and the infinite words by $\sigma\in\Sigma^{\omega}$.}
\begin{definition}[Feasible words $\sigma_i\in\Sigma_i$]\label{defn:infTSi}
A word $\sigma_i\in\Sigma_i$ is \textit{feasible} if and only if $\sigma_i\not\models b_j^{\text{inf}}$, where $b_j^{\text{inf}}$ is a Boolean formula defined as 
\begin{equation}\label{bInfTSi}
b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e}(\pi_j^{r_i}\wedge\pi_j^{r_e})).
%b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e})).
\end{equation}
\end{definition}

Note that the Boolean formula $b_j^{\text{inf}}$ is satisfied by any finite word $\sigma_j\in\Sigma_j$ that requires robot $j$ to be present in two or more disjoint regions, simultaneously. For instance, the word $\sigma_j=\pi_j^{r_i}\pi_j^{r_e}$ satisfies $b_j^{\text{inf}}$.\footnote{Note that if we consider regions $r_i$ that are not necessarily disjoint, then the Boolean formula $b_j^{\text{inf}}$ is defined as $b_j^{\text{inf}}=\vee_{\forall r_i}( \vee_{\forall r_e \text{s.t.} r_i \cap r_e=\emptyset} (\pi_j^{r_i}\wedge\pi_j^{r_e}))$. Note also that definition of infeasible words depends on the problem at hand, i.e, the definition of atomic propositions included in the sets $\mathcal{AP}_j$.} % if there is an overlap between regions $r_i$ and $r_e$. 
Next, we define the feasible words $\sigma\in\Sigma$.

\begin{definition}[Feasible words $\sigma\in\Sigma$]\label{defn:infPTS}
A word $\sigma\in\Sigma$ is \textit{feasible} if and only if $\sigma_j\not\models b_j^{\text{inf}}$, for all robots $i$,
where $\sigma_j=\Pi|_{\Sigma_j}\sigma$, $b_j^{\text{inf}}$ is defined in \eqref{bInfTSi}, and $\Pi|_{\Sigma_j}\sigma$ stands for the projection of the word $\sigma$ onto $\Sigma_j=2^{\mathcal{AP}_j}$.\footnote{For instance, $\Pi|_{\Sigma_j}(\pi_j^{r_e}\pi_m^{r_h})=\pi_j^{r_e}$.}
\end{definition}

Then we define the feasible DFA transitions as follows
\begin{definition}[Feasible DFA transitions]
A transition $(q_D,\sigma^*,q_D')\in\rightarrow_D$ is feasible if the finite word $\sigma\in\Sigma=2^{\mathcal{AP}}$ is a \textit{feasible} word .%and (ii) there exists at least one pair of words $\sigma_{\text{inv}}$ and $\sigma_{\text{next}}$, such $\Pi|_{\Sigma_j} \sigma_{\text{inv}}=\Pi|_{\Sigma_j} \sigma_{\text{inv}}$, for all robots $j$ for which $\Pi|_{\Sigma_j} \sigma_{\text{inv}}$ is non-empty.
\end{definition}

%\begin{ex}~[DFA transitions]
%For instance, a DFA transition from $q_D$ to $q_D'$ under the following conditions $b_{\text{inv}}^{q_D}=\pi_j^{r_i}$ and $b_{\text{next}}^{q_D,q_D'}=\pi_j^{r_i}\wedge \pi_m^{r_h}$ is feasible. On the other hand, if the Boolean formulas $b_{\text{inv}}^{q_D}$ and $b_{\text{next}}^{q_D,q_D'}$ are  $b_{\text{inv}}^{q_D}=\pi_j^{r_i}$ and $b_{\text{next}}^{q_D,q_D'}=\pi_j^{r_e}\wedge \pi_m^{r_h}$, then the transition from $q_D$ to $q_D'$ is infeasible, since this would require robot $j$ to instaneously move from $r_i$ to $r_e$ which is not possible given that $r_i$ to $r_e$ are disjoint regions.
%\end{ex}



Then, on the pruned DFA, we define a function $d:\ccalQ_D\times\ccalQ_D\rightarrow \mathbb{N}$ that returns the minimum number of \textit{feasible} DFA transitions that are required to reach a state $q_D'\in\ccalQ_D$ starting from a state $q_D\in\ccalQ_D$. This function will be used to guide the robots towards locations in the workspace so that eventually a final DFA state is visited, i.e., the LTL formula is satisfied.
%
Particularly, we define the distance function $d: \ccalQ_D \times \ccalQ_D \rightarrow \mathbb{N}$ as follows
\begin{equation}
d(q_D,q_D')=\left\{
                \begin{array}{ll}
                  |SP_{q_D,q_D'}|, \mbox{if $SP_{q_D,q_D'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_D,q_D'}$ denotes the shortest path (in terms of hops) in the  pruned DFA from $q_D$ to $q_D'$ and $|SP_{q_D,q_D'}|$ stands for its cost (number of hops).

\subsection{Selecting a Feasible DFA Final State}\label{sec:feasFinal}
Given the pruned DFA, the distance function, and an initial DFA state $q_D(0)$, our next step is to select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, i.e., a final state that is reachable from $q_D(0)$ in the pruned DFA [line \ref{rrt:feasFinal}, Alg. \ref{alg:RRT}]. In math, given an initial state  $q_D(0)$ feasible final states are the ones that satisfy  $d(q_D(0),q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. If there do not exist such final states given the state $q_D(0)$, then we select another initial DFA state $q_D(0)$ from $\ccalQ_D^0$. If there do not exist initial states such that $d(q_D^0,q_{F})\neq \infty$, then the LTL formula can not be satisfied and an error message is returned.



%Next at any time $t\geq 0$, given the current DFA state $q_D(t)$, we select a target DFA state, denoted by $q_D^{\text{target}}$, that the robots should reach next. This state is selected so that it is one hop closer to $q_F^{\text{feas}}$ than $q_D(t)$ is, i.e.,

The pruning step and the selection of a feasible final state are part of the initialization of Algorithm \ref{alg:RRT}; see Section \ref{sec:prune}-\ref{sec:feasFinal}. In what follows, we present the online part of Algorithm \ref{alg:RRT}; see Sections \ref{sec:targetDFA}-\ref{sec:paths}.

\subsection{Selecting a Target DFA State}\label{sec:targetDFA}
Given the current robot positions $\bbp_j(t)$  and the current DFA state $\bbq_d(t)$ at time $t\geq 0$, every robot $j$ needs to locally design a path $\bbp_{j,t:T_j}$ that if followed by all robots $j$ , the distance of $q_D(T)$ from the feasible final state $q_F^{\text{feas}}$ is less than the distance of the current DFA state $q_D(t)$ from $q_F^{\text{feas}}$. To this end, we select a target DFA state, denoted by $q_D^{\text{target}}$, that the robots should reach at time $T$, i.e.,
$q_D(T)=q_D^{\text{target}}$ as follows. First, we compute the distance $d(q_D(t),q_F^{\text{feas}})$. Then, we select as $q_D^{\text{target}}$ the state that satisfies 
\begin{equation}\label{eq:targetDFA}
   d(q_D^{\text{target}},q_F^{\text{feas}}) = d(q_D(t),q_F^{\text{feas}}) -1, 
\end{equation}
i.e., a state that is one hop closer to $q_F^{\text{feas}}$ than $q_D(t)$ is. If there are more than one states that satisfy \eqref{eq:targetDFA}, we select one randomly. 

The state $q_D^{\text{target}}$ is updated when the robots either reach it or realize that a transition from $q_D(t)$ to $q_D^{\text{target}}$ is in fact infeasible; see next section.




\subsection{Distributed Online Construction of Robot Paths}\label{sec:paths}
Given the target DFA state $q_D^{\text{target}}$, our goal is to design paths $\bbp_{j,t:T}$ that when executed, the DFA transition from $q_D(t)$ to $q_D^{\text{target}}$ will be activated. To achieve that, it suffices to ensure that the robot paths (i) always satisfy the invariant condition that allows the robot to stay in the current DFA state and (ii) never satisfy properties that enable DFA transitions to DFA states $q_D'\neq q_D(t)$ and $q_D'\neq q_D^{\text{target}}$ Both (i) and (ii) should hold until (iii) the condition that enables transition from $q_D(t)$ to $q_D^{\text{target}}$ is satisfied. %Once (iii) becomes true, (iv) the invariant condition that allows the robot to stay in $q_D^{\text{target}}$ should also be satisfied at the same time. The latter condition ensures that a feasible path originating from $q_D^{\text{target}}$ can be designed \red{[i think you dont need that, if not feasible then next operator exists...]}; see also Section \ref{sec:complOpt}.

To formally state these requirements, we introduce the following definitions and notations. First, we define the Boolean formula $b_{\text{inv}}$ which if satisfied by the multi-robot state $\bbp(t)$, i.e., if $\bbp(t)\models b_{\text{inv}}$, then the robots remain in the same DFA state, i.e., $\bbq_D(t)=\delta(L(\bbp(t)),\bbq_D(t))$. %We also denote $b_{\text{inv}}^{\text{target}}$ the corresponding invariant condition for $q_D^{\text{target}}$.
%
Moreover, we denote by $b_{\text{target}}$ and $b_{\text{others}}$ the Boolean formulas that if satisfied, then the DFA transitions from $q_{D}(t)$ to $q_D^{\text{target}}$ and from $q_{D}(t)$ $q_D'$ are enabled respectively, where $q_D'\neq q_{D}(t)$ and $q_D'\neq q_D^{\text{target}}$. 

Given the above definitions, a centralized approach to design paths $\bbp_{j,t:T}$, for all robots $j$, that satisfy the desired properties (i)-(iii) discussed above would be to use available temporal logic motion planners [\red{cite}] to synthesize paths that satisfy the following LTL property that captures conditions (i)-(iii).
%
\begin{equation}
    \phi_{\text{target}}= %(\Diamond b_{\text{target}})\wedge 
    \underbrace{(b_{\text{inv}} \ccalU b_{\text{target}} )}_{\text{(i)}~\&~\text{(iii)}} \wedge  \underbrace{(\neg b_{\text{others}} \ccalU b_{\text{target}})}_{\text{(ii)}~\&~\text{(iii)}}.%\wedge  \underbrace{(b_{\text{target}}\to b_{\text{inv}}^{\text{target}})}_{\text{(iv)}}.
\end{equation}
%
Nevertheless, such approaches do not scale well with the size of the robots. Temporal logic planning algorithms for large-scale multi-robot systems have also been proposed but their runtime increases as the number of robots increases which is undesirable in the considered problem set-up where re-planning may be required as the environment is discovered. 

Motivated by this limitation, we propose a distributed temporal logic planning algorithm that allows the robots to locally design paths $\bbp_{j,t:T_j}$, for some $T_j>t$, that once executed the DFA state $q_D^{\text{target}}$ will be reached. %Note that construction of these paths occurs locally and does not require communication between robots. %However, their execution requires communication between robots; see Section \ref{sec:exec}. 
To this end, we first re-write the Boolean  formula $b_{\text{target}}$ so that we separate the atomic propositions that appear with a negation operator in front of them from those that the negation operator does not exist. Specifically, we re-write $b_{\text{target}}$ as follows
%\begin{equation}
%    b_{\text{target}} = b_{\text{target}}^{\text{goal}} \wedge (\neg \bar{b}_{\text{target}}^{\text{goal}} )
%\end{equation}
%
\begin{equation}\label{eq:target1}
    b_{\text{target}} = b_{\text{target}}^{\text{goal}} \triangle (\neg b_{\text{target}}^{\text{avoid}} ),
\end{equation}
where in both Boolean formulas $b_{\text{target}}^{\text{goal}}$ and $b_{\text{target}}^{\text{avoid}}$ the negation operator does not appear in front of any atomic proposition. Also, in \eqref{eq:target1}, $\triangle$ denotes either the logical AND ($\wedge$) or the logical OR $(\vee)$ operator; see also Example \ref{ex1}.% and $\bar{b}_{\text{target}}^{\text{goal}}$ the 


Next, we decompose $b_{\text{target}}^{\text{avoid}}$ as follows
\begin{equation}\label{eq:avoid}
    b_{\text{target}}^{\text{avoid}}= (\vee_j b_{\text{target},j}^{\text{avoid}}) \triangle b_{\text{target,all}}^{\text{avoid}}
\end{equation}
where $b_{\text{target},j}^{\text{avoid}}$ is a Boolean formula defined over $\mathcal{AP}_j$, i.e., that can be satisfied exclusively by robot $j$; see also Example \ref{ex2}. Similarly, $b_{\text{target,all}}^{\text{avoid}}$ is a Boolean formula defined over $\mathcal{AP} = \cup_j\mathcal{AP}_j$, i.e., it cannot be satisfied by a single robot. 


Observe in \eqref{eq:avoid} that the formulas $b_{\text{target},j}^{\text{avoid}}$ are coupled with each other with the logical OR operator, since a formula of the form $b_{\text{target},j}^{\text{avoid}}\wedge b_{\text{target},e}^{\text{avoid}}$ is part of  $b_{\text{target,all}}^{\text{avoid}}$ by definition. % of atomic propositions associated only with robot $j$ (coupled with each other through the conjunction and/or disjunction operator) while 

Next, we select a word $\sigma_{\text{target}}$ that satisfies $b_{\text{target}}$, i.e., $\sigma\models b_{\text{target}}$; see also Example \ref{ex3}. Among all \text{feasible} words, we select the one with the minimum length. Given $\sigma_{\text{target}}$, we compute the region, denoted by $L_j^{\text{target}}$ that robot $j$ has to be located, so that if all robots $j$ are at their corresponding locations $L_j^{\text{target}}$, then the word $\sigma$ is generated and $b_{\text{target}}$ is satisfied.  If $\triangle$ in \eqref{eq:target1} is the logical AND, then we collect in a set $\ccalA_j^{\text{target}}$ the regions that if robot $j$ visits then $b_{\text{target},j}^{\text{avoid}}$ is satisfied and, therefore, $b_{\text{target}}$ is violated regardless of the positions of the other robots. On the other hand, if $\triangle$ in \eqref{eq:target1} is the logical OR, then $\ccalA_j^{\text{target}}=\emptyset$. \red{[explain why]}
%If $\triangle$ in \eqref{eq:target1} is the logical AND, then

\begin{ex}[Decomposition of $b_{\text{target}}$]\label{ex1}
For instance, the Boolean formula
\begin{equation}\label{eq:example}
    b_{\text{target}}=(\pi_j^{r_1}\vee \pi_j^{r_3} )\wedge\pi_e^{r_2}\wedge (\neg \pi_j^{r_2}) \wedge (\neg (\pi_j^{r_1}\wedge \pi_e^{r_1})).
\end{equation}
can be rewritten as in \eqref{eq:target1} by defining the following subformulas:
\begin{equation}\label{eq:example_cnt1}
    b_{\text{target}}^{\text{goal}}=(\pi_j^{r_1}\vee \pi_j^{r_3})\wedge\pi_e^{r_2}
\end{equation}
and 
\begin{equation}\label{eq:example_cnt2}
    b_{\text{target}}^{\text{avoid}}=\pi_j^{r_2} \vee (\pi_j^{r_1}\wedge \pi_e^{r_1})
\end{equation}
\end{ex}

\begin{ex}[Decomposition of $b_{\text{target}}^{\text{avoid}}$]\label{ex2}
For instance, for the Boolean formula $b_{\text{target}}^{\text{avoid}}$ in \eqref{eq:example_cnt2}, we have that 
\begin{align}\label{eq:avoid1}
    &b_{\text{target},j}^{\text{avoid}}= \pi_j^{r_2}\nonumber\\
    &b_{\text{target},e}^{\text{avoid}}=\varnothing\\
    &b_{\text{target,all}}^{\text{avoid}}=\pi_j^{r_1}\wedge \pi_e^{r_1}\nonumber
\end{align}
\end{ex}

\begin{ex}[Satisfaction of $b_{\text{target}}^{\text{goal}}$]\label{ex3}
For instance, a word $\sigma_{\text{target}}$ that satisfies \eqref{eq:example} is $\sigma_{\text{target}}=\pi_j^{r_1}\pi_e^{r_2}$. Given this word, we have that $L_j^{\text{target}}=r_1$ and $L_e^{\text{target}}=r_2$. Also, given the formulas $b_{\text{target},j}^{\text{avoid}}$ and $b_{\text{target},e}^{\text{avoid}}$ in \eqref{eq:avoid1}, we have that $\ccalA_j^{\text{target}}=r_2$ and $\ccalA_e^{\text{target}}=\emptyset$.
\end{ex}

We follow the same decomposition steps for the Boolean formula $b_{\text{inv}}$ as well. Given $b_{\text{inv}}$, we can similarly (i) construct the set $\ccalA_j^{\text{inv}}$ and (ii) select the word $\sigma_{\text{inv}}$ with the minimum length that satisfies $b_{\text{inv}}$, i.e., $\sigma_{\text{inv}} \models b_{\text{inv}}$. 

Given $\sigma_{\text{inv}}$ and  $\sigma_{\text{target}}$, we design paths $\bbp_{j,t:T_j}$ that will satisfy the conditions (i)-(iii) that were previously discussed. Specifically, the robots need to generate the word $\sigma_{\text{target}}$ to reach $q_D^{\text{target}}$. While navigating the environment so that they generate $\sigma_{\text{target}}$ we need to ensure that $b_{\text{inv}}$ is always satisfied which guarantees that robots can stay in $q_D(t)$. Note that if the later does not hold, the robots may reach a state $q_D'\neq q_D^{\text{target}}$ from which $q_D^{\text{target}}$ may not be reachable. We design such paths as follows. First, all robots that are involved in generating $\sigma_{\text{inv}}$, collected in a set $\ccalR_{\text{inv}}$, stay idle at their current locations $\bbp_j(t)$, i.e., $T_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$. In Section \ref{sec:complOpt}, we show that if robots collected in the set $\ccalR_{\text{inv}}$ already generate the word $\sigma_{\text{inv}}$, and, therefore, they do not need to move towards other regions. 
%
All other robots $j\notin\ccalR_{\text{inv}}$ solve the following local optimal control problems to design their paths $\bbp_{j,t:\bar{T}_j}$ that if followed the word  $\sigma_{\text{target}}\models b_{\text{target}}$ will be generated and the DFA state $q_D^{\text{target}}$ will be reached.

\begin{subequations}
\label{eq:localProb}
\begin{align}
& \min_{\substack{T_j, \bbu_{t:T_j}}} \left[J(T_j,\bbu_{t:T_j}) = \sum_{t'=t}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \cup_i \{r_i\}\setminus R_j(t), \forall t'\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{target}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin \ccalA_j^{\text{avoid}} \label{constrLoc2}\\
& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
\end{align}
\end{subequations}
where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. If it does not lie in any of the regions $r_i$, then $R_j(t)=\varnothing$. Also, the first constraint \eqref{constrLoc1} requires that robot $j$ should not visit any region $r_i$ excluding the region $R_j(t)$ (if it is defined), for all time instants until the time instant $T_j$ when robot $j$ should be in region $L_j^{\text{target}}$. The later is captured by the second constraint in \eqref{constrLoc2} and is required in order to generate the word $\sigma_{\text{target}}$. In words, the optimal control problem \eqref{eq:localProb} requires robot $j$ to design a path $\bbp_{j,t:T_j}$ with the minimum horizon $T_j$ that reaches $L_j^{\text{target}}$ while avoiding all regions $r_i$ excluding the region $R_j(t)$. Note that the robots that do not belong to $\ccalR_{\text{inv}}$ and also are not responsible to generate $\sigma_{\text{target}}$ do not have a target region $L_{j}^{\text{target}}$. These robots remain stationary to their current locations and they do not need to solve \eqref{eq:localProb}.
%
Observe that \eqref{eq:localProb} is a deterministic shortest path problem, and, therefore, any of the traditional motion planning algorithms, such as $\text{A}^*$, RRT, $\text{RRT}^*$, RRG, or PRM, can be used to solve it. Finally observe that robot $j$ locally solves \eqref{eq:localProb} without communicating with any other robot. %Feasibility of such this problem is examined in 

%We design such paths in two stages. In the first stage, we design subpaths $\bbp_{j,t:\bar{T}_j}$ for some $t<\bar{T}_j<T$ and in the second stage we design paths $\bbp_{j,\bar{T}_j:T_j}$. In particular, \textit{in the first stage} all robots that are involved in generating $\sigma_{\text{inv}}$, collected in a set $\ccalR_{\text{inv}}$, and all other robots $j$ for which it hold $L(\bbp_j(t))=\varnothing$ (i.e., they are outside of all regions $r_i$) stay idle at their current locations $\bbp_j(t)$, i.e., $\bar{T}_j=t+1$ and $\bbp_{j,t:\bar{T}_j}=[\bbp_j(t),\bbp_j(t)]$ All other robots $j$ (i.e., the ones that satisfy $j\notin\ccalR_{\text{inv}}$ and $L(\bbp_j(t))\neq \varnothing$) solve the following optimal control problem to design paths $\bbp_{j,t:\bar{T}_j}$ that if followed then the robots will move outside the regions that they are currently located. %As it will bbe discusses in Section \ref{sec:exec}, these subpaths will be executed so that the robots will move outside their current regions simultaneously.

%\begin{subequations}
%\label{eq:localProb1}
%\begin{align}
%& \min_{\substack{\bar{T}_j, \bbu_{t:\bar{T}_j}}} \left[J(\bar{T}_j,\bbu_{t:\bar{T}_j}) = \sum_{t'=t}^{\bar{T}_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc1}\\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in R_j(t), \forall t\in\set{t,\dots,\bar{T}_j-1} \label{constrLoc1a} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\in \ccalR_j^{\text{inv}}, \forall t\in\set{t,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   L(\bbp_j(\bar{T}_j))=\varnothing \label{constrLoc2a}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   %\bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc2}
%\end{align}
%\end{subequations}
%where $R_j(t)$ denotes the region $r_i$ that robot $j$ lies in at time $t$. Observe that the first two constraints \eqref{constrLoc1a}-\eqref{constrLoc2a} require robot $j$ to move outside the region $\ccalR_j(t)$ where it is located at the time instant $t$. This happens at a time instant $\bar{T}_j$, i.e., $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that robot $j$ locally solves \label{eq:localProb1} with communicating with other robots. Observe that execution of these subpaths ensures that the robots remain in the DFA state $q_D(t)$ since $b_{\text{inv}}$ is always satisfied as the robots $\ccalR_{\text{inv}}$ remain stationary in their current locations that generates  $\sigma_{\text{inv}}\models b_{\text{inv}}$.

%since the robots in $\ccalR_{\text{inv}}$

%In the \textit{second} stage, we construct the subpaths $\bbp_{j,\bar{T}_j:T_j}$ that will enable the transition from $q_D(t)$ to $q_D^{\text{target}}$. For robots $j\in\ccalR_{\text{inv}}$, we select $T_j=\bar{T}_j+1$ and $\bbp_{j,\bar{T}_j:T_j}=[\bbp_{j}(t),\bbp_{j}(t)]$, i.e., these robots still stay idle. In fact, due to the deterministic structure of the DFA, this ensures that the robots remain in the DFA state $q_D(t)$ until the word $\sigma_{\text{target}}$ is generated which will activate the transition towards $q_D^{\text{target}}$. To generate the word  $\sigma_{\text{target}}$, all other robots $j\notin\ccalR_{\text{inv}}$ design paths $\bbp_{j,\bar{T}_j:T_j}$ by solving the following optimal control problem:

%\begin{subequations}
%\label{eq:localProb}
%\begin{align}
%& \min_{\substack{T_j, \bbu_{\bar{T}_j:T_j}}} \left[J(T_j,\bbu_{\bar{T}_j:T_j}) = \sum_{t'=\bar{T}_j}^{T_j}  w(\bbp_j(t'),\bbp_j(t'+1)) \right] \label{ObjLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \ L(\bbp_j(t'))=\varnothing, \forall t'\in\set{\bar{T}_j,\dots,T_j-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \ \bbp_j(t')\notin \ccalA_j^{\text{inv}}, \forall t\in\set{T,\dots,\bar{T}-1} \label{constrLoc1} \\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\in L_j^{\text{target}} \label{constrLoc2}\\
%\in (L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})
%
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(T_j)\notin %\ccalA_j^{\text{avoid}} \label{constrLoc2}\\
%& \ \ \ \ \ \ \ \ \ \ \   \bbp_j(t'+1)=\bbf_j(\bbp_j(t'),\bbu_j(t')), \label{constrLoc3}
%\end{align}
%\end{subequations}



 %This ensures that  transition to a DFA state $q_D'\neq q_D(t)$ that is not $q_D^{\text{target}}$. 
%In the meantime the robots in $\ccalR_{\text{inv}}$ ensure that the current DFA state remain the same in $[t,\bar{T}-1]$, since they stay idle and generate the word $\sigma_{\text{inv}}$. Also note that robots in $\ccalR_{\text{inv}}$ do not belong to the set of robots that need to move to another location to generate the word $\sigma$, since that would create a conflict; see also Remark \ref{rem:invariant}. 
%The second constraint in \eqref{constrLoc2} requires that at time instant $T_j$, all robots should be in their corresponding locations $L_j^\textbf{}$. Once this happens the word $\sigma_{\text{target}}$ is generated and the target DFA state is reached.
%



Moreover, observe that the local optimal control problem \eqref{eq:localProb} may be \textit{infeasible}. This can be the case e.g., if the region $L_j^{\text{target}}$ is surrounded by obstacles or because of the robot dynamics. In this case, robot $j$ needs to communicate with all other robots so that a new feasible word $\sigma_{\text{target}}$ is selected. This process is repeated until regions $L_j^{\text{target}}$ are selected that make \eqref{eq:localProb} feasible. If such a word $\sigma$ does not exist, then this means that the transition from $q_D(t)$ to $q_D^{\text{target}}$ is infeasible, given the current multi-robot state $\bbp(t)$. Then, the pruned DFA is updated by removing this transition. Next, a new target DFA state is selected that satisfies \eqref{eq:targetDFA}. If there do not exist such DFA states then this means that the selected final state $q_F^{\text{feas}}$ is not \text{feasible}. In this case, another final state is selected to be $q_F^{\text{feas}}$ that is reachable from $q_D(t)$. If there do not exist any feasible final states, then the robots cannot accomplish the assigned task and the mission needs to be restarted. Note that this does not necessarily mean that there do not exist paths that satisfy the assigned LTL specification. In fact, there may exist another sequence of DFA states for which the optimal control problem \eqref{eq:localProb} is always feasible; see also Section \ref{sec:complOpt}. Conditions under which \eqref{eq:localProb} is always feasible and, therefore, Algorithm \ref{alg:RRT} is complete, are provided in Section \ref{sec:complOpt}. %Note that infeasibility of \eqref{eq:localProb} is due to the facts (i) the environment is unknown and, therefore, it is not possible to check offline which DFA transitions cannot be enabled because e.g., of the robot dynamics or the existence of obstacles.%; and (ii) the LTL formula $\phi$ is decomposed into local sub-tasks Problem \ref{prob} is solved in a distributed the proposed algorithm is distributed nature of the proposed 

%What if the problem is infeasible? update $\sigma$ i.e., $L_j$. If no other $L_j$. update target DFA state. If no other target DFA state report `current method failed (this does not mean that the task is unsatisfiable though)'

\subsection{Asynchronous Execution of Paths}\label{sec:exec}
%Let $\ccalR_{\sigma}$ denote the set of robots that are responsible for generating the word $\sigma$. 
%First, the robots execute the subpaths $\bbp_{j,t:T_j}$. Specifically, 
%The robots that design $\bbp_{j,t:T_j}$ as per the solution of \eqref{eq:localProb}, execute \textit{asynchronously} their paths until the time instant $\bar{T}_j-1$, i.e., right before they step out of their respective regions $R_j(t)$. Then, every robot $j$ waits for all other robots $e$ with $\bar{T}_e>\bar{T}_j$. At the time instant $\bar{T}=\max_{j} \bar{T}_j-1$ when all robots have reached the penultimate waypoint of their paths $\bbp_{j,t:\bar{T}_j}$, they \textit{synchronously} move towards the last waypoint of $\bbp_{j,t:\bar{T}_j}$ that satisfies $L(\bbp_j(\bar{T}_j))=\varnothing$. Note that if we allow the robots to move asynchronously outside their respective regions $R_j(t)$, then words $\sigma$ may be generated that enable a transition to a state $q_D'\neq q_D(t)$ and  $q_D'\neq q_D^{\text{target}}$. On the other hand, since the robots move outside these regions synchronously, this guarantees that in the time interval $[t,\max_j \bar{T}_j]$ the robots remain in the DFA state $q_D(t)$. 


The robots that design $\bbp_{j,t:T_j}$ as per the solution of \eqref{eq:localProb}, execute \textit{asynchronously} their paths until the time instant $T_j-1$, i.e., right before these robots step into their respective target regions $L_j^{\text{target}}$.
Then, every robot $j$ waits for all other robots $e$ with $T_e>T_j$. At the time instant $T=\max_{j} T_j-1$, i.e., when all robots have reached the penultimate waypoint of their paths $\bbp_{j,\bar{T}_j,T_j}$, they \textit{synchronously} move towards the last waypoint of $\bbp_{j,t:\bar{T}_j}$ that satisfies $\bbp_j(T_j)\in\L_j^{\text{target}}$ and the word $\sigma_{\text{target}}$ is generated. Note that during the time interval $[t, \max_j{T_j}-1]$, the robots remain in the DFA state $q_D(t)$ and at $\max_j{T_j}$ the word $\sigma_{\text{target}}$ is generated and transition from $q_D(t)$ to $q_D^{\text{target}}$ occurs; see Section \ref{sec:complOpt}.

%Note that by construction and execution of the paths $\bbp_{j,t:T_j}$, we get that the global Boolean subformulas \red{...} are never satisfied which would violate the LTL specification

%Note that the construction of paths $\bbp_{j,t:T_j}$ as per \eqref{eq:localProb} ignores the global subformulas $b_{\text{target,all}}^{\text{avoid}}$ and $b_{\text{inv,all}}^{\text{avoid}}$ that depend on the global state $\bbp(t)$ of the multi-robot system. Recall that these formulas should never be satisfied, as this would mean that the LTL-specified task $\phi$ is violated. As a result, it is possible that there exist time instants $t'$ such that state $\bbp(t')$ violates $\phi$. To mitigate this issue, we require all robots $j$ to communicate with each other at all time instants $t'\in\set{t,\dots,T_j-1}$ to check if their next global position $\bbp_j(t'+1)$ satisfies the Boolean formula $b_{\text{inv,all}}^{\text{avoid}}$. If this is the case, the robots coordinate with each other to check which robots can move first towards their next position $\bbp_{j}(t+1)$ and which ones will stay put at the current time instant so that $b_{\text{inv,all}}^{\text{avoid}}$ is not satisfied. Note that this requires an exhaustive search over all possible combinations until a successful combination is found. In case none of these combinations is valid, then the proposed algorithm cannot satisfy the assigned LTL property.  %Alternatively, centralized temporal logic planning algorithms can be employed to re-synthesize a team plan. 

%At time $t=T_j-1$, i.e., at the time instant before robot $j$ stepping in the region $(L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})$ (by construction of \eqref{eq:localProb}), every robot $j$ waits until the time instant $\max T_e-1$, when all robots associated with the word $\sigma$ are about to to visit their respective assigned locations $L_e$. Once, this happens, all robots synchronously move towards their corresponding locations to generate the word that will enable the DFA transition to the state $q_D^{\text{target}}$. In fact, a robot $j$ can wait inside the region $(L_j\cap \ccalR_j)\setminus (\ccalA_j^{\text{inv,target}}\cup \ccalA_j^{\text{avoid}})$ for the other robots (i.e., before generating the word $\sigma$) assuming that this does not violate the Boolean formula $b_{\text{inv}}$.  As discussed before, it is possible that the state $\bbp(T)$ violates the global subformula $\bar{b}_{\text{target,all}}^{\text{goal}}$ and in this case the LTL property is not satisfied.

%Nevertheless, in practice the global Boolean formulas $b_{\text{target,all}}^{\text{avoid}}$ and $b_{\text{inv,all}}^{\text{avoid}}$ are often quite hard to satisfy, especially for large number of robots and/or small regions $r_i$, as they require specific robots to be at specific locations simultaneously; this is was also validated in our simulation studies. As a result, we can also allow the robots to move asynchronously, without communicating with each other, until the time instants $\min T_j$.



%Note that the locations $\bbp_j(t)$ of the robots $j\in\ccalR_{\text{inv}}$ already ensure that $\sigma_{\text{inv}}$ that $b_{\text{inv}}$ holds; see also Remark \ref{rem:invariant}. All other robots $j$ that also satisfy $L(\bbp_j(t))\neq \varnothing$ (i.e., they are inside a region $r_i$) solve the following optimal control problem to design paths $\bbp_{j,t:T}$ that will let them get out of the regions that they are currently located, at the same time $T$, for some $T>t$.


%Note that by construction of the paths $\bbp_{j,t:T}$, we have that in the time interval $[t,T]$, the Boolean formula $b_{\text{inv}}$ is satisfied. Therefore, due to the deterministic structure of the DFA, we have that $q_D(t)=q_D(T)$, i.e., the DFA state does not change during the time interval $[t,T]$. Then, at time $T$, the robots design paths $\bbp_{j,T:T_j}$ that if followed the state $q_D^{\text{target}}$ will be reached. This is accomplished by following the optimal control problem.




%
\begin{rem}\label{rem:invariant}
Note that once the robots reach a new DFA $q_D$, they satisfy its respective Boolean condition $b_{\text{inv}}$, since the `next' temporal operator is excluded from the task specification. Particularly, if $b_{\text{inv}}$ is not satisfied this implies that once the robots are at locations that generate a word that triggers the transition to $q_D$, the robots should immediately leave their locations, which is impossible to specify unless the next operator is included in the specification language. 

Recall that $\sigma_{\text{inv}}$ is selected to have the minimum length, this means that the minimum number of robots are involved to generate it. Therefore, robots that are required to generate the word $\sigma$ are not included in the set $\ccalR_{\text{inv}}$; see also Remark \ref{rem:invariant}.
Similarly, robots that are responsible to satisfy $b_{\text{target}}$ cannot be responsible for generating the word $\sigma_{\text{inv}}$, since the next operator does not exist and all regions are assumed to be disjoint. %(unless there is an overlap..)
\end{rem}






%and $b_{\text{others}}$,% and $\ccalA_j^{\text{others}}$. %The same notations extend to $b_{\text{inv}}$ and $b_{\text{others}}$.
%\begin{equation}
%    b_{\text{inv}} = b_{\text{inv}}^{\text{goal}} \wedge (\neg \bar{b}_{\text{inv}}^{\text{goal}} )
%\end{equation}
%where in both Boolean formulas $b_{\text{inv}} = b_{\text{inv}}^{\text{goal}}$ and $\bar{b}_{\text{inv}}^{\text{goal}}$ the negation operator does not appear in front of any atomic proposition.% and $\bar{b}_{\text{inv}}^{\text{goal}}$ the 
%
%Next, we express $\bar{b}_{\text{inv}}^{\text{goal}}$ as follows
%\begin{equation}
%    \bar{b}_{\text{inv}}^{\text{goal}}= (\vee_j \bar{b}_{\text{inv},j}^{\text{goal}}) \vee \bar{b}_{\text{inv,all}}^{\text{goal}},
%\end{equation}
%where
%
%Then, we collect in a set $\ccalA_j^{\text{inv}}$ the regions $r_i$ that if visited by robot $j$, then  $b_{\text{inv},j}^{\text{avoid}}$ is satisfied, which means that $b_{\text{inv}}$ is violated (regardless of the state of other robots). Similarly, we collect in the set $\ccalA_j^{\text{others}}$ the regions that satisfy the formula $b_{\text{others},j}^{\text{goal}}$. 
%Also, we collect in the sets $\ccalR_j$ and $\ccalA_j^{\text{inv,target}}$ the regions that satisfy $b_{\text{inv,target},j}^\text{goal}$ and $b_{\text{inv,target},j}^\text{avoid}$. Typically, $b_{\text{inv,target}}$ requires all robots to avoid obstacles and in this case $\ccalR_j$ and $\ccalA_j^{\text{inv,target}}$ correspond to the obstacle-free and obstacle space, respectively.
%
%We perform exactly the same steps for $\bar{b}_{\text{others}}=\neg b_{\text{others}}$ and we collect the corresponding regions in a set denoted by $\ccalA_j^{\text{others}}$.
%Next, we define the set $\ccalA_j=\ccalA_j^{\text{inv}}\cup \ccalA_j^{\text{others}}$ that collects all regions that robot $j$ should avoid. [\red{give example}]

%Similarly, we re-write
%\begin{equation}
%    b_{\text{target}} = b_{\text{target}}^{\text{goal}} \wedge (\neg \bar{b}_{\text{target}}^{\text{goal}} )
%\end{equation}
%and we further decompose $\bar{b}_{\text{target}}^{\text{goal}}$ as



\subsection{Online Re-planning}\label{sec:replan}
As the robots follow their paths $\bbp_{j,t:T_j}$, they may discover new obstacles based on their sensor measurements; see \eqref{eq:sensor}. If the discovered obstacles intersect with a path $\bbp_{j,t:T_j}$, then that robot $j$ needs updates the set $\ccalA_j$ of locations that it should avoid and re-solves \eqref{eq:localProb} to design a new path. 

%Next, we define the set $\ccalL_j$ that collects all robot positions $\bbp_j$ that violate $b_{\text{inv}}$ regardless of the state of all other robots. For instance, if $b_{\text{inv}}=\neg (\pi_j^{r_e}\wedge \pi_z^{r_h})$, then $\ccalL_j=\emptyset$. On the other hand, if $b_{\text{inv}}=\neg (\pi_j^{r_e})\wedge (\neg \pi_z^{r_h})$ then  $\ccalL_j=\set{r_e}$. Formally, to construct the set, we express the negation of $b_{\text{inv}}$, denoted by $\bar{b}_{\text{inv}}=\neg b_{\text{inv}}$ as




==> files/extensionsLDBA.tex <==
In Section \ref{sec:planning}, we proposed an RL algorithm that exploits an automaton-based representation of LTL formulas to accelerate the training process. Specifically, the proposed biased exploration strategy relies on translating LTL formulas into DRA. In this section, we show that the proposed exploration stategy can be extended to Limit Deterministic B\"uchi Automaton (LDBA) that typically have a smaller state space than that of DRA which can further accelerate the learning process \cite{hasanbeig2018logically}. In Section \ref{sec:LDBA}, we define the LDBA and in Section \ref{sec:theoryLDBA}, we present a LDBA-based reward structure that guarantees that maximizing accumulated rewards (see \eqref{eq:policy0}) is equivalent to maximizing the satisfaction probability (see \eqref{eq:xistar}) \cite{hasanbeig2019reinforcement}. Finally, in Section \ref{sec:biasedLDBA} we discuss how the biased policy can be constructed.

\subsection{Translating LTL into an LDBA}\label{sec:LDBA}
Converting an LTL formula into a DRA results, in the worst case, in automata that are doubly exponential in the size of the original LTL formula \cite{dra4}. Motivated by this, recent works employ LDBA to represent LTL formulas \cite{hasanbeig2018logically, hasanbeig2019reinforcement, bozkurt2020control} which is more succinct automaton~\cite{sickert,sickert2}. This results in reducing the state-space that needs to be explored. 

Before defining the LDBA, we first need to define the Generalized B\"uchi Automaton (GBA).
\begin{definition}[Generalized B\"uchi Automaton \cite{baier2008principles}]
A GBA $\mathfrak{A} = (\ccalQ, q_0, \Sigma, \ccalF, \delta)$ is a structure where $\ccalQ$ is a finite set of states, $q_0\in\ccalQ$ is the initial state, $\Sigma=2^{\mathcal{AP}}$ is a finite alphabet, $\ccalF = {\ccalF_1,\dots, \ccalF_f }$ is the set of accepting conditions where $\ccalF_j \subset\ccalQ$, $1\leq j \leq f$, and $\delta:\ccalQ\times\Sigma\rightarrow 2^{\ccalQ}$ is a transition relation. $\hfill\Box$ 
\end{definition}

An infinite run $\rho$ of $\mathfrak{A}$ over an infinite word $\sigma=\pi_0\pi_1\pi_2\dots\in\Sigma^{\omega}$, $\pi_k\in\Sigma=2^{\mathcal{AP}}$ $\forall k\in\mathbb{N}$, is an infinite sequence of states $q_k\in\ccalQ$, i.e.,  $\rho=q_0q_1\dots q_k\dots$, such that $q_{k+1}\in\delta(q_k,\pi_k)$. The infinite run $\rho$ is called \textit{accepting} (and the respective word $\sigma$ is accepted by the GBA) if $\texttt{Inf}(\rho)\cap\ccalF_j\neq\emptyset,\forall j\in\set{1,\dots,f},$ %   
%\begin{equation}\label{acc}
%\texttt{Inf}(\rho)\cap\ccalF_j\neq\emptyset,\forall j\in\set{1,\dots,f},     
%\end{equation}
where $\texttt{Inf}(\rho)$ is the set of states that are visited infinitely often by $\rho$. 
%there exists at least one pair $(\ccalG_i,\ccalB_i)$ such that $\texttt{Inf}(\rho_D)\cap\ccalG_i\neq\varnothing$  and $\texttt{Inf}(\rho_D)\cap\ccalB_i=\varnothing$, where $\texttt{Inf}(\rho_B)$ represents the set of states that appear in $\rho_D$ infinitely often.

%\emergencystretch 3em
%\sloppy
%\RaggedRight
\begin{definition}[Limit Deterministic B\"uchi Automaton \cite{sickert}]\label{ldbadef}
A GBA $\mathfrak{A} = (\ccalQ, q_0, \Sigma, \ccalF, \delta)$ is {\it limit deterministic} if
$\ccalQ$ can be partitioned into two disjoint sets $\ccalQ = \ccalQ_N \cup \ccalQ_D$, so that (i) $\delta(q,\pi)\subset\ccalQ_D$ and $|\delta(q,\pi)|=1$, for every state $q\in\ccalQ_D$ and $\pi\in\Sigma$; and (ii) for every $\ccalF_j\in\ccalF$, it holds that $\ccalF_j\subset\ccalQ_D$
%\begin{itemize}
%    \item $\delta(q,\pi)\subset\ccalQ_D$ and $|\delta(q,\pi)|=1$, for every state $q\in\ccalQ_D$ and $\pi\in\Sigma$,
%    \item for every $\ccalF_j\in\ccalF$, $\ccalF_j\subset\ccalQ_D$,
%\end{itemize}
and there are $\varepsilon$-transitions from $\ccalQ_N$ to $\ccalQ_D$. $\hfill\Box$ 
\end{definition}

An $\varepsilon$-transition allows the automaton to change its state without reading any specific input. In practice, the $\varepsilon$-transitions between $ \mathcal{Q}_N $ and $ \mathcal{Q}_D $ reflect the ``guess'' on reaching $ \mathcal{Q}_D $: accordingly, if after an $\varepsilon$-transition the associated labels in the accepting set of the automaton cannot be read, or if the accepting states cannot be visited, then the guess is deemed to be wrong, and the trace is disregarded and is not accepted by the automaton. However, if the trace is accepting, then the trace will stay in $\mathcal{Q}_D$ ever after, i.e. $\mathcal{Q}_D$ is invariant. 


\subsection{LDBA-based reward assignment}\label{sec:theoryLDBA}

Given an (non-pruned) LDBA, we construct the product MDP, i.e., the product between the MDP and the LDBA. The formal definition of this PMDP can be found in \cite{bozkurt2020control, hasanbeig2018logically}. 
To synthesize a policy that satisfies the LDBA accepting conditions,  we adopt the synchronous reward function for the product MDP proposed in \cite{hasanbeig2018logically}. The main idea is that (i) visiting a set $\ccalF_j$, $1\leq j\leq f$ yields a positive reward $r>0$; and (ii) revisiting the same set $\ccalF_j$ returns zero reward until all other sets $\ccalF_k$, $k\neq j$ are also visited; (iii) the rest of the transitions have zero rewards. Intuitively, this reward shaping strategy motivates the agent to visit \textit{all} accepting sets $\ccalF_j$ of the LDBA infinitely often, as required by the acceptance condition of the LDBA. We note that any other reward function can be used, as e.g., the one in \cite{bozkurt2020control} that is supported by probabilistic satisfaction guarantees as well.

\subsection{Biased LDBA-based Exploration}\label{sec:biasedLDBA}
Once the LDBA is constructed, it is pruned exactly as the DRA is pruned \ref{sec:prune}. The $\epsilon$-transitions are not pruned. Given the pruned automaton, similar to \eqref{eq:dist2G}, we define the distance to an accepting set of states $\ccalF_j$ as follows

\begin{equation}\label{eq:dist2G2}
    d_F(q,\ccalF_j)=\min_{q_G\in\ccalF_j} d(q,q_G)
\end{equation}
where $d(q,q_G)$ is defined as in \eqref{eq:dist1}. This distance function is used to bias exploration so that each set $\ccalF_j$ is visited infinitely often. Note that the main difference between the accepting conditions of the LDBA and the DRA is that the former requires to visit all accepting sets infinitely often while the latter requires to visit at least one accepting set infinitely often. To design a biased exploration strategy that can account for the LDBA accepting condition, we first define the set $\ccalV$ that collects indices $j$ to the set of accepting states $\ccalF_j$ that have not been visited during the current RL episode. Then, among all non-visited set of accepting states $\ccalF_j$, we pick one randomly based on which we define the set $\ccalQ_{\text{goal}}(q_{\text{cur}})$. Similar to \eqref{eq:Qnext}, we define the set $\ccalQ_{\text{goal}}(q_{\text{cur}})$ as follows:

%
\begin{align}\label{eq:Qnext2}
    \ccalQ_{\text{goal}}(q_{\text{cur}})=&\{q'\in\ccalQ~|~(\exists\sigma\in\Sigma_{\text{feas}}~\text{such that}~q'\in\delta(q_{\text{cur}},\sigma))\nonumber\\& \wedge (d_F(q',\ccalF_j)=d_F(q_{\text{cur}},\ccalF_j)-1)\},
\end{align}
where $j\in\ccalV$. Recall, that all $\epsilon$- transitions in the LDBA are feasible. Thus, in \eqref{eq:Qnext2}, $ \ccalQ_{\text{goal}}(q_{\text{cur}})$ includes all states $q'$ where the transition from $q_{\text{cur}}$ to $q$ is an $\epsilon$-transition. Given $ \ccalQ_{\text{goal}}(q_{\text{cur}})$, the biased action is selected exactly as described in Section \ref{sec:biasedExpl}. Once the set of states $\ccalF_j$ is visited, the set $\ccalV$ is updated as $\ccalV=\ccalV\setminus\{j\}$, and then the set $\ccalQ_{\text{goal}}(q_{\text{cur}})$ is updated accordingly.





==> files/parallel.tex <==
\subsection{Parallel Design of Sample-Efficient Control Policies}

Given the initial robot states, our goal is to design a control policy that will drive the robots to the final DRA state. To this end, we first need to define the set $\ccalX_{q_D}$, for each state $q_D$, that collects all product MDP states that the robots should be located in order to reach $q_D$. Construction of this set can be accomplished by inspecting the conditions under which transitions from states $q_D'\neq q_D$ to $q_D$, in the pruned DRA, can be enabled. For instance, assume that $N=2$ and a state $q_D$ can be reached in one hop only from states $q_D^1$ and $q_D^2$ under if the following Boolean formulas are satisfied respectively: $b_1=\pi_{q_1^e}\wedge \pi_{q_2^w}$ and $b_1=\pi_{q_1^r}\vee \pi_{q_2^e}$. In this case, the set $\ccalX_{q_D}$ is defined as $\ccalX_{q_D}=\{(q_1^e,q_2^w),(q_1^r,\cdot),(\cdot,q_2^e),(q_1^r,q_2^e)\}$. \red{[this set is well defined, i.e. there are not case a state that requires robot i to be in more than two states simulatnaeously exist, by pruning of DRA.]}

Then to design a control policy $\boldsymbol{\xi}$ that solves Problem \ref{prob}, we first design control policies $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow(\bbx',q_D')}$ that will drive the robots from the product MDP state $\bbx$ and DRA state $q_D$ to the product MDP state $\bbx'$ and DRA state $q_D'$, where $\bbx\in\ccalX_{q_D}$ and $\bbx'\in\ccalX_{q_D}'$. Also, it holds that $d(q_D',q_F) = d(q_D,q_F) -1$ by construction of the DRA. This process is repeated, in parallel, for all $\bbx\in\ccalX_{q_D}$ and $\bbx'\in\ccalX_{q_D}'$ and for all pairs of states $q_D$ and $q_D'$, where $q_D'$ is reachable within one hop from $q_D$ in the pruned DRA. Computation of a control policy $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow(\bbx',q_D')}$ is described in Algorithm \ref{alg:RL-LTL}. A policy $\boldsymbol{\xi}$ that solves Problem \ref{prob} will be computed by composing the policies $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow(\bbx',q_D')}$.

%Given the current robot MDP states and the current DRA state, denoted by  $x_j^{\text{cur}}$ and $\bbq_D^{\text{cur}}$ respectively, our goal is to design control policies that will drive the robots to DRA  states that are closer to the final state $q_F$ than the current DRA state $q_D^{\text{cur}}$ is. To this end, we collect all such DRA states in the set
%\begin{equation}
%    \ccalQ_{\text{next}}^{q_D^{\text{cur}}}=\{q_D'|d(q_D',q_F) = d(q_D^{\text{cur}},q_F) -1\}. 
%\end{equation}



%To synthesize such a policy, we first select a state that belongs to $\ccalQ_{\text{next}}^{q_D}$, denoted by $q_D^{\text{next}}$. The following process is repeated for all states $q_D^{\text{next}}\in \ccalQ_{\text{next}}^{q_D}$. 

%\begin{definition}[PMDP]
%...
%in this product MDP all states that observe something else other than sigmanext are obstacles'/sinks
%...
%\end{definition}

In what follows, we propose a sample-efficient Q-learning approach to design control policies $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow(\bbx',q_D')}$. To achieve that, we first define a reward function for the product MDP so that (i) visiting the state $\bbx'$ of the product MDP, yields a positive reward $\alpha>0$, since $\delta_D(\bbq_D,L(\bbx'))=q_D'$; (ii) visiting any other PMDP state $\bbx'$ yields a zero reward. %that satisfies $L(\bbx)\neq \varnothing$
%Intuitively, this reward strategy motivates the robots to visit their respective MDP states that will trigger the transition to one of the states $\ccalQ_{\text{next}}^{q_D}$ while avoiding all sink states. Formally, we define the reward function as,
%
%(ii) visiting any other state $\bbx$ that satisfies $L(\bbx)\neq \varnothing$ yields a negative reward $\beta<0$; (iii) the rest of the transitions have negative rewards $0\geq\gamma>\beta$. Intuitively,  this reward strategy motivates the agent to visit the state $\bbx$ that will trigger the transition to one of the states $\ccalQ_{\text{next}}^{q_D}$ by following the shortest path (see (i) and (iii)), while avoiding all regions that may yield transitions to DRA states $q_D'\neq q_D$ (see (ii)). 
Formally, we define the reward function as follows:

\begin{equation}\label{def:prodRewMDPi}
\begin{aligned}
R_{(\bbx,q_D)\rightarrow (\bbx',q_D')}(\bbx^{\text{cur}},\bba) = \left\{
\begin{array}{lr}
\alpha>0 & \text{if}~\bbx^{\text{next}} = \bbx',\\
0 & \text{otherwise}.
\end{array}
\right.
\end{aligned}
\end{equation}
where $\bbx^{\text{next}}$ is a state that is reached from $\bbx^{\text{cur}}$ after applying the control action $\bba$. Hereafter, when it is clear from the context, with slight abuse of notation, we simply denote $R_{(\bbx,q_D)\rightarrow (\bbx',q_D')}(\bbx^{\text{cur}},\bba)$ by $R(\bbx^{\text{cur}},\bba)$.

Given the PMDP $\mathfrak{P}$, we compute a \textit{stationary deterministic} policy $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow(\bbx',q_D')}^*$ (which, for simplicity, is also denoted by $\boldsymbol\mu^*$), that maximizes the expected accumulated return, i.e.,

\begin{equation}\label{eq:policy0}
	\boldsymbol\mu^*(\bbx)=\arg\max\limits_{\boldsymbol\mu \in \mathfrak{D}}~ {U}^{\boldsymbol\mu}(\bbx),
\end{equation}
%where $\mathfrak{D}$ is the set of all stationary deterministic policies over $\mathcal{S}$, and 	
\begin{equation}\label{eq:utility}
{U}^{\boldsymbol\mu}(\bbx)=\mathbb{E}^{\boldsymbol\mu}[\sum\limits_{k=0}^{\infty} \gamma^k~ R(\bbx_t,\boldsymbol\mu(\bbx_t))|\bbx_0=\bbx],
\end{equation}
%where $\mathbb{E}^{\boldsymbol\mu} [\cdot]$ denotes the expected value given that the product MDP follows the policy $\boldsymbol\mu$ \cite{puterman}, $\gamma$ is the discount factor, and $s_0,...,s_n$ is the sequence of states generated by policy $\boldsymbol\mu$ up to time step $n$, initialized at $s_0 = s$. Note that the optimal policy is stationary as shown in the following result.

\begin{theorem}[\!\!\cite{puterman}]
In any finite-state MDP, such as $\mathfrak{P}$, if there exists an optimal policy, then that policy is stationary and deterministic. $\hfill\Box$
\end{theorem}

In order to construct $\boldsymbol\mu^*$, we employ episodic Q-learning (QL), a model-based RL algorithm described in Algorithm~\ref{alg:RL-LTL}.\footnote{Note that any other model-based RL algorithm can also be used within Algorithm~\ref{alg:RL-LTL}, including any variant of the class of temporal difference learning algorithms~\cite{sutton}.} Specifically, Algorithm \ref{alg:RL-LTL} requires as inputs (i) the reward function $R$ defined in \eqref{def:prodRewMDPi}, and (ii) the hyper-parameters of the learning algorithm. 
%
The action-value function $Q(\bbx,\bba)$ and the model for robot $j$ (i.e., the MDP transition probabilities) $P_j(x_j,a,x_j')$ can be initialized arbitrarily. Note that $U^{\boldsymbol\mu}(\bbx)=\max_{\bba \in \mathcal{A}_\mathfrak{P}}Q(\bbx,\bba)$. Also, we define a function $n_j:\mathcal{X}_j\times\mathcal{A}_j\rightarrow\mathbb{N}$ that counts the number of times that action $a$ has been taken by robot $j$ at state $x_j$. Similarly, we define $c_j :\mathcal{X}_j\times\mathcal{A}_j\times\ccalX_j\rightarrow\mathbb{N}$ that counts the number of times that robot $j$ visited state $x_j'$ after taking action $a$ at state $x_j$. This pair of functions is required to estimate the transition probabilities $P_j(x_j,a,x_j')$. As a policy, we propose an extension of the $\epsilon$-greedy policy, called $(\epsilon,\delta)$-greedy policy that selects an action $\bba$ at state $\bbx$ by using the learned action-value function $Q$ (as the standard $\epsilon$-greedy policy) and the learned dynamics $P_j$. Specifically, according to this policy, with probability $(1-\epsilon)$, the greedy action $\argmax_{\bba\in\mathcal{A}_\mathfrak{P}}Q(\bbx,\bba)$ is taken while with probability $\epsilon\times\delta$ an random action $\bba$ is selected. Also, with probability $\epsilon\times\delta$ all robots select a random action. 
%
Finally, with probability $\epsilon\times(1-\delta)$ each robot $j$ locally selects at state $x_j$ the action $a_j$ that has the maximum likelihood of leading it to a state $x_j'$ that is closer to a state $x_j^{\text{next}}$ that robot $j$ needs to visit so that a symbol $\sigma_{\text{next}}$ that is required to transition to the DRA state in $q_D^{\text{next}}$, is generated. Formally, $(\epsilon,\delta)$-greedy policy $\boldsymbol{\pi}$ is defined as

%Specifically, to compute this action, the robots first randomly select a state $q_D'\in\ccalQ_{q_D}$

\begin{equation*}
\boldsymbol{\pi}(\bbx,\bba) = \begin{cases}
1-\epsilon &\text{if ~}  \bba=\max_{\bba' \in \mathcal{A}_\mathfrak{P}}Q(\bbx,\bba')\\
\epsilon\times\delta  &\text{if}~\bba \in \mathcal{A}_\mathfrak{P}\\
\epsilon\times(1-\delta) &\text{if ~} \bba=\bar{\bba}
\end{cases}
\end{equation*}
where the action $\bar{\bba}$ is computed as follows. First, robot $j$, for each action $a_j$  computes 
\begin{equation}
x_j^{a_j}=\argmax_{x_j'} P_j(x_j,a_j,:),
\end{equation}
which denotes the most likely state for robot $j$ to end up after taking action $a_j$ at state $x_j$ based on the learned dynamics captured by $P_j$. This is repeated all actions $a_j\in\ccalA_j$ and the resulting states are collected in the set $\bar{\ccalX}_j$. Among all states in $\bar{\ccalX}_j$, we collect in the set $\bar{\ccalX}_j^{\text{closer}}$ the states $x_j^{a_j}$ that are closer to $x_j^{\text{next}}$ than the current state $x_j$ is. The corresponding actions $a_j$ are collected in the set $\ccalA_j^{\text{closer}}$. Then, the action $\bar{\bba}$ is defined as $\bar{\bba}=[\bar{a}_1,\dots,\bar{a}_N]$, where

\begin{equation}
    \bar{a}_j = \argmax_{a_j} \{P_j(x_j,a_j,x_j^{a_j})\}_{\forall a_j\in \ccalA_j^{\text{closer}}}
\end{equation}
i.e., $\bar{a}_j$ is the action with maximum likelihood of driving the robot to state (in one hop) that is closer to $x_j^{\text{next}}$.

Every episode terminates when the robots either reach the goal state $\bbx'$ that enables the transition from $q_D$ to $q_D'$ or visit a state that belongs to a set $\mathcal{X}_{\text{avoid}}\subseteq\ccalX$ defined as follows:

\begin{equation}\label{eq:avoid}
    \mathcal{X}_{\text{avoid}} = \set{\bar{\bbx}\in\ccalX\setminus\set{\bbx'}~|~  \delta_D(q_D,L(\bar{\bbx}))\neq q_D}
\end{equation}
%L(\bar{\bbx})=\text{`obstacle'} \vee

In words, $\mathcal{X}_{\text{avoid}}$ collects all states $\bar{\bbx}$ (excluding the state $\bbx'$) that if visited, then a transition to a DRA state $\bar{q}_D\neq q_D$ will be enabled. This also means that even states (excluding the goal state $\bbx^g$) that may enable a transition to $q_D'$ are included in $\mathcal{X}_{\text{avoid}}$. Also obstacle-states are also included in $\mathcal{X}_{\text{avoid}}$, since if visited the robots cannot stay in $q_D$, as in this case $\phi$ is violated. This way, the robots are motivated to reach the DRA state by observing $L(\bbx^g)$ while avoiding regions that may also enable a transition to $q_D^g$ or to any other DRA state.

Once all $Q_{(\bbx,q_D)\rightarrow (\bbx',q_D')}$ functions have converged and the policies $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow (\bbx',q_D')}^*$ have been learned, we synthesize the policy $\boldsymbol\xi$ as follows. First, we create a weighted graph whose set of nodes is indexed by pairs $(\bbx, q_D)$ and edges from $(\bbx, q_D)$ to $(\bbx', q_D')$ exist for each learned policy $\boldsymbol{\mu}_{(\bbx,q_D)\rightarrow (\bbx',q_D')}^*$. The weight on the each edge is the optimal state-action value i.e., $Q_{(\bbx,q_D)\rightarrow (\bbx',q_D')}(\bbx,\boldsymbol{\mu}^*)$ while the cost of a path $\bbq=(\bbx^0,q_D^0),(\bbx^1,q_D^1),\dots,(\bbx^K,q_D^K)$ is  $C_\bbq =\prod_{k=0}^{K-1} Q_{(\bbx^k,q_D^k)\rightarrow (\bbx^k,q_D^{k+1})}$. As it will be shown in Section \ref{sec:theory}, $Q_{(\bbx,q_D)\rightarrow (\bbx',q_D')}(\bbx,\boldsymbol{\mu}^*)$ represents the probability of observing $L(\bbx^g)$ which triggers transition to $q_D^g$ while avoiding regions/observations that may either enable a transition to $q_D^g$ or to any other DRA state. Thus, $Q_{(\bbx,q_D)\rightarrow (\bbx',q_D')}(\bbx,\boldsymbol{\mu}^*)$ is a lower bound of reaching of the probability of reaching the DRA state $q_D^g$ starting from the PMDP state $\bbx^g$ and the DRA state $q_D^g$. Thus, $C_{\bbq}$ acts a lower bound of the satisfaction probability of $\phi$, since there can be multi paths/observations to reach a state $q_D$ from $q_D'$. \red{[the last sentence is possibly wrong...?]} 

Then, in $\ccalG$, we compute the longest path $\bbq=(\bbx^0,q_D^0),(\bbx^1,q_D^1),\dots,(\bbx^K,q_D^K)$ (i.e., the path with the highest cost $C_\bbq$) that connects that $(\bbx^0,q_D^0)$ to a state $(\cdot,q_F)$. Then, policy $\boldsymbol{\xi}$ is constructed by concatenating the control policies $\boldsymbol{\mu}_{(\bbx^k,q_D^k)\rightarrow (\bbx^{k+1},q_D^{k+1})}^*$, where $(\bbx^k,q_D^k)$ are determined by the path $\bbq$. Note that as the robot navigates the workspace as per $\boldsymbol{\mu}_{(\bbx^k,q_D^k)\rightarrow (\bbx^{k+1},q_D^{k+1})}^*$, where $(\bbx^k,q_D^k)$, a state $(\bbx',q_D')$ maybe reached due to uncertainty, instead of the desired state $(\bbx^{k+1},q_D^{k+1})$. In this case, $\boldsymbol\xi$ is re-synthesized by computing the longest path in $\ccalG$ that connects  $(\bbx',q_D')$ to $(\cdot,q_F)$.


\begin{rem}
Note that as $\epsilon\rightarrow 0$, it holds that $\boldsymbol\mu$ asymptotically converges to the optimal greedy policy $\boldsymbol\mu^*=\argmax_{a\in\mathcal{A}_\mathfrak{P}} Q^*(\bbx,\bba)$, where $Q^*$ is the optimal $Q$ function. Further, $Q(\bbx,\boldsymbol\mu^*(\bbx))=U^{\boldsymbol\mu^*}(\bbx)=V^*({\bbx})$, where $V^*({\bbx})$ is the optimal value function that could have been computed via Dynamic Programming (DP) if the MDP was fully known \cite{sutton,reachability_in_hybrid,cont_pctl}. 
\end{rem}%Projection of $\boldsymbol\mu^*$ onto the state-space of the PL-MDP, yields the finite-memory policy $\boldsymbol\xi^*$ that solves Problem \ref{pr:pr1}.

%the current DRA state of the multi-robot system becomes $q_D^{\text{cur}}=q_D^{\text{next}}$, and the above process is repeated until the final state is reached. This way, a policy $\boldsymbol{\xi}_{\bbq}$ can be learned to drive the robot from an initial state $q_D^0$ to $q_F$ through a specific sequence of DRA states $\bbq=q_D^0,q_D^1,\dots,q_K$, where $q_K=q_F$. In Section \ref{sec:theory}, we show that $\boldsymbol{\xi}_{\bbq}\models\phi$ with probability $\prod_{k=0}^{K-1} Q_{q_D^k\rightarrow q_D^{k+1}}$. Thus, after computing policies $\boldsymbol{\xi}_{\bbq}$ for all possible paths $\bbq$ that connect $q_D^0$ to $q_F$ in the pruned DRA, we select the policy with the maximum satisfaction probability as a solution to Problem \ref{prob}.

%\subsubsection{Parallel RL for LTL Planning}

%Recall that to compute $\boldsymbol{\xi}_{\bbq}$, control policies $\boldsymbol{\pi}_{q_D^k\rightarrow q_D^{k+1}}$ need to be computed sequentially, which can become computationally expensive for large paths $\bbq$. In this section, we show that all control policies $\boldsymbol{\pi}_{q_D\rightarrow q_D'}$ can be computed in parallel which can significantly speed up the learning process.


\begin{algorithm}[t]
%\footnotesize
\caption{Sample-Efficient RL for LTL planning}
\LinesNumbered
\label{alg:RL-LTL2}
\KwIn{ (i) initial robot configuration $\bbx(0)$, (ii) LTL formula $\phi$}
Initialize $Q_{q_D}(\bbx,a)$ and $P$ arbitrarily, $n(\bbx,a)=0$, $\bbx^\text{cur}=\bbx^0$\;
$\pi_{q_D}=(\epsilon,\delta)-\text{greedy}(Q_{q_D})$\;
\While{$Q_{q_D}$ has not converged}{
%\texttt{terminate}=0\;
\While{($L(q_D,\bbx^{\text{next}})\notin\ccalQ_{\text{next}}^{q_D}$) OR ($L(q_D,\bbx^{\text{next}})\neq\text{'obstacle'}$)}{
Pick action $\bba^\text{cur}$ from $\pi_{q_D}$\; 
Observe $\bbx^{\text{next}}$, and $R(\bbx^\text{cur},\bba^{\text{cur}},\bbx^\text{next})$\;
%\If{($L(q_D,\bbx^{\text{next}})\in\ccalQ_{\text{next}}^{q_D}$) OR ($L(q_D,\bbx^{\text{next}})=\text{'obstacle'}$)}{
%\texttt{terminate}=1\;}
$\bbx^\text{cur}=\bbx^\text{next}$\;
Update $\epsilon$\;
%
$n(x_j^{\text{cur}},a_j^{\text{cur}})=n(x_j^{\text{cur}},a_j^{\text{cur}})+1$\;
$c(x_j^{\text{cur}},a_j^{\text{cur}},x_j^{\text{next}})=c(x_j^{\text{cur}},a_j^{\text{cur}},x_j^{\text{next}})+1$\;
Update model $P_j(x_j^{\text{cur}},a_j^{\text{cur}},x_j^{\text{next}})=c(x_j^{\text{cur}},a_j^{\text{cur}},x_j^{\text{next}})/n(x_j^{\text{cur}},a_j^{\text{cur}})$\;
%
$Q_{q_D}(\bbx^\text{cur},\bba^{\text{cur}})= Q_{q_D}(\bbx^\text{cur},\bba^{\text{cur}})+(1/n(\bbx^\text{cur},\bba^{\text{cur}}))[R(\bbx^\text{cur},\bba^{\text{cur}})-Q_{q_D}(\bbx^\text{cur},\bba^{\text{cur}})+\gamma \max_{\bba'}(\bbx^{\text{next}},\bba'))]$\;
Update set of MDP states that are occupied by obstacles\;}}
\end{algorithm}



 %or realize that a transition from $q_D(t)$ to $q_D^{\text{target}}$ is in fact infeasible; see next section.


==> files/proofs1.tex <==
To prove Theorem \ref{thm:sampleEf}, we need first to introduce the following proposition. Then in Section \ref{sec:mainP1}, we provide the detailed proof of Theorem \ref{thm:sampleEf}. %In what follows, we assume that the the MDP transition probabilities are accurately known, i.e., $P(x,a,x')=\hat{P}(x,a,x')$, for all MDP transitions. Relaxation of this assumption is discussed later in the section. %Here, by progress towards accomplishing the LTL task, we mean that for the next product MDP state $s_{\text{after}}=(x_{\text{after}},q_{\text{after}})$ during the RL episode, it holds that %$J_{x_{\text{cur}}$

%that the next product MDP state denoted by $s_{\text{after}}$ is one-hop closer to a set of product states 


%and $s_{\text{after}}\in\ccalR_{\mathfrak{P}}(s_{\text{cur}})$. Let also $x_b\in\ccalX_{\text{closer}}(x_{\text{cur}})$ denote the MDP state towards which the action $a_b$ is biased.


\begin{prop}\label{prop:sampleEf1}%%[Comparative Sample Efficiency]
Let $s_{\text{cur}}=(x_{\text{cur}},q_{\text{cur}})$ be  the product MDP state at the current RL episode/iteration of Algorithm \ref{alg:RL-LTL}. %$s_{\text{cur}}=(x_{\text{cur}},q_{\text{cur}})$ be the state reached at the next iteration of the current RL episode. 
Let also $x_b\in\ccalX_{\text{closer}}(x_{\text{cur}})$ denote the MDP state towards which the action $a_b$ is biased. If \eqref{eq:AsAvP} holds,
%\begin{equation}\label{eq:AsAvP}
%    P(x_{\text{cur}},a_b,x_b)>\sum_{a\in\ccalA(x_{\text{cur}})}\frac{P(x_{\text{cur}},a,x)}{|\ccalA(x_{\text{cur}})|}, \forall x\in\ccalX_{\text{closer}}(x_{\text{cur}}),
%\end{equation}
%for all $x\in\ccalX_{\text{closer}}(x_{\text{cur}})$, 
then 
\begin{equation}\label{eq:compSample}
    \mathbb{P}_b(x_{\text{after}}\in\ccalX_{\text{closer}}(x_{\text{cur}}))> \mathbb{P}_g(x_{\text{after}}\in\ccalX_{\text{closer}}(x_{\text{cur}})),
\end{equation}
where $\mathbb{P}_g(x_{\text{after}}\in\ccalX_{\text{closer}})$ and $\mathbb{P}_b(x_{\text{after}}\in\ccalX_{\text{closer}})$ denote the probability of reaching at the next iteration of the current RL episode any state $x_{\text{after}}$ that belongs to $\ccalX_{\text{closer}}(x_{\text{cur}})$ starting from $x_{\text{cur}}$ without and with bias introduced in the exploration phase, respectively.
\end{prop}


\begin{proof}
The probability of reaching a state $s_{\text{after}}=(x_{\text{after}},q_{\text{after}})$ where $x_{\text{after}}\in\ccalX_{\text{closer}}$ under a policy $\boldsymbol\mu(s)$ is: $$\sum_{x\in\ccalX_{\text{closer}})}\sum_{a\in\ccalA(x_{\text{cur}})}\boldsymbol\mu(s_{\text{cur}},a)P(x_{\text{cur}},a,x).$$ Thus, we have that:
\begin{align}\label{eq:diff1}
    &\mathbb{P}_b(x_{\text{after}}\in\ccalX_{\text{closer}})- \mathbb{P}_g(x_{\text{after}}\in\ccalX_{\text{closer}})=\\&\sum_{x\in\ccalX_{\text{closer}}(x_{\text{cur}})}\sum_{a\in\ccalA(x_{\text{cur}})}P(x_{\text{cur}},a,x)(\boldsymbol\mu_b(s_{\text{cur}},a)-\boldsymbol\mu_g(s_{\text{cur}},a)), \nonumber
\end{align}
where $\boldsymbol\mu_g$ and $\boldsymbol\mu_b$ refer to the $\epsilon$-greedy (no biased exploration) and $(\epsilon,\delta)$-greedy policy (biased exploration), respectively.
In what follows, we compute $\boldsymbol\mu_b(s_{\text{cur}},a)-\boldsymbol\mu_\epsilon(s_{\text{cur}},a)$, for all $a\in\ccalA_{\mathfrak{P}}$. Recall, that $\boldsymbol\mu_b(s_{\text{cur}},a)$ is the probability of selecting the action $a$ at state $s_{\text{cur}}$. Also, hereafter, we assume that the greedy action $a^*$ is different from the biased action $a_b$; however, the same logic applies if $a_b=a^*$, leading to the same result .

First, for the action $a=a^*$, we have that
\begin{align}\label{eq:mua*}
    &\boldsymbol\mu_b(s_{\text{cur}},a^*)-\boldsymbol\mu_g(s_{\text{cur}},a^*)\nonumber\\&=(1-\epsilon+\frac{\delta_e}{m})-(1-\epsilon +\frac{\epsilon}{m})\nonumber\\&=(1-\epsilon+\frac{\delta_e}{m})-(1-\epsilon +\frac{\delta_b+\delta_e}{m})\nonumber\\&=\frac{\delta_b}{m}.
\end{align}
Similarly, for $a=a_b$, we have that
\begin{align}\label{eq:muab}
    &\boldsymbol\mu_b(s_{\text{cur}},a_b)-\boldsymbol\mu_g(s_{\text{cur}},a_b)=(\delta_b+\frac{\delta_e}{m})-\frac{\epsilon}{m}\nonumber\\&=-\frac{\delta_b(m-1)}{m}.
\end{align}
Also, for all other actions $a\neq a_b,a^*$, we have that
\begin{align}\label{eq:mua}
    &\boldsymbol\mu_b(s_{\text{cur}},a)-\boldsymbol\mu_g(s_{\text{cur}},a)=\frac{\delta_e}{m}-\frac{\epsilon}{m}\nonumber\\&=-\frac{\delta_b}{m}.
\end{align}
Substituting \eqref{eq:mua*}-\eqref{eq:mua} into \eqref{eq:diff1} yields:
\begin{align}\label{eq:diff2}
    &\mathbb{P}_b(x_{\text{after}}\in\ccalX_{\text{closer}})- \mathbb{P}_g(x_{\text{after}}\in\ccalX_{\text{closer}})=\nonumber\\&\sum_{x\in\ccalX_{\text{closer}}}\left(P(x_{\text{cur}},a_b,x_b)\delta_b-\sum_{a\in\ccalA(x_{\text{cur}})}P(x_{\text{cur}},a,x)\frac{\delta_b}{m}\right)=\nonumber\\&\delta_b\sum_{x\in\ccalX_{\text{closer}}}\left(P(x_{\text{cur}},a_b,x_b)-\sum_{a\in\ccalA(x_{\text{cur}})}\frac{P(x_{\text{cur}},a,x)}{m}\right).
\end{align}
Due to \eqref{eq:AsAvP}, we conclude that $\mathbb{P}_b(s_{\text{after}}\in\ccalX_{\text{closer}})- \mathbb{P}_g(s_{\text{after}}\in\ccalX_{\text{closer}})>0$ completing the proof.
\end{proof}

\begin{rem}
Observe that \eqref{eq:compSample} may hold even if assumption \eqref{eq:AsAvP} does not hold for all MDP states $x\in\ccalX_{\text{closer}}$ (see \eqref{eq:diff2}). Nevertheless, \eqref{eq:AsAvP} always holds for the MDP state $x_b\in\ccalX_{\text{closer}}$, if the MDP transition probabilities have been learned accurately enough. The reason is that by definition of the action $a_b$ in \eqref{eq:a_b}, it holds that $P(x_{\text{cur}},a_b,x_b)>P(x_{\text{cur}},a,x_b)$, for all $a\in A_{\mathfrak{P}}$ and, therefore, $P(x_{\text{cur}},a_b,x_b)$ must be greater than the average of all probabilities $P(x_{\text{cur}},a,x_b)$. This equivalently means that if $|\ccalQ_{\text{next}}|=1$ and $|\ccalX_{\text{closer}}|=1$ (i.e., $|\ccalX_{\text{closer}}|=\{x_b\}$), then \eqref{eq:AsAvP} holds by definition of $a_b$, and, therefore, \eqref{eq:compSample} holds as well.
\end{rem}

\subsection{Main Proof}\label{sec:mainP1}
Using Proposition \ref{prop:sampleEf1}, in what follows we provide the proof of Theorem \ref{thm:sampleEf}.
%
%\begin{proof}
%Let $s_{\text{after}}^k$ denote be the current product state of the robot during an RL episode, i.e., $s_{\text{cur}} = s_{\text{after}}^k$. 
In words we want to show that the probability of reaching a DRA state in $\ccalQ_{\text{goal}}(q_{\text{cur}})$ within the minimum number of iterations from $s_{\text{cur}}$ (i.e., within $k^*=J_{x_{\text{cur}},\ccalX_{\text{goal}}}$ iterations) is higher when bias is introduced in the exploration phase. To shows this, it suffices to show that the probability of reaching the states in $\ccalX_{\text{goal}}(q_{\text{cur}})$ that are $k^*$ hops from $x_{\text{cur}}$ while always avoiding MDP states belonging to $\ccalX_{\text{avoid}}$ %that can enable a transition from $q_{\text{cur}}=q_{\text{after}}^k$ to any other DRA state 
(see Remark \ref{rem:shortestPath}) is higher when bias is introduced; note that there may be states in $\ccalX_{\text{goal}}(q_{\text{cur}})$ that are more than $k^*$ hops from $x_{\text{cur}}$. The reason is that once a state in $\ccalX_{\text{goal}}(q_{\text{cur}})$ is reached a transition from $q_{\text{cur}}$ to a state in $\ccalQ_{\text{goal}}(q_{\text{cur}})$ is enabled by definition of $\ccalX_{\text{goal}}(q_{\text{cur}})$.
%
To describe this statement in math, we need to introduce the following definitions. 

Let $\bar{\ccalX}\subseteq\ccalX$ be set of MDP states. Then, we define
\begin{equation}\label{eq:def1}
    \ccalX_{\text{closer}}(\bar{\ccalX})=\bigcup_{x\in\bar{\ccalX}}\ccalX_{\text{closer}}(x).
\end{equation}
Based on \eqref{eq:def1}, we define the following set:
\begin{equation}\label{eq:def2}
    \ccalX_{\text{closer}}^2(x_{\text{cur}}) := \ccalX_{\text{closer}}(\ccalX_{\text{closer}}(x_{\text{cur}}))=\bigcup_{x\in\ccalX_{\text{closer}}(x_{\text{cur}})}\ccalX_{\text{closer}}(x).
\end{equation}
By applying \eqref{eq:def2} recursively we can define the set $$ \ccalX_{\text{closer}}^n(x_{\text{cur}}):=\ccalX_{\text{closer}}(\ccalX_{\text{closer}}^{n-1}(x_{\text{cur}})),$$ for all $n\geq2$. Observe that $ \ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})\subseteq \ccalX_{\text{goal}}(q_{\text{cur}})$. By definition of the set $\ccalX_{\text{closer}}^n(x_{\text{cur}})$, we have that $\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})\subseteq \ccalX_{\text{goal}}(q_{\text{cur}})$, since $\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})$ collects the states in $\ccalX_{\text{goal}}(q_{\text{cur}})$ that are $k^*$ hops from $x_{\text{cur}}$. Also, note that by construction of the shortest paths (see Remark \ref{rem:shortestPath}), we have that the set $\ccalX_{\text{closer}}^{k^*-1}(x_{\text{cur}})$ 
% =x_{\text{after}^k}
does not include any MDP states $x$ that can enable a transition from $q_{\text{cur}}=q_{\text{after}}^k$ to any other DRA state. Thus, we get that
\begin{align}
    &\mathbb{P}_b(q_{\text{after}}^{k+k^*+1}\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}})\nonumber\\&=\mathbb{P}_b(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}}),
\end{align}
and
\begin{align}
    &\mathbb{P}_g(q_{\text{after}}^{k+k^*+1}\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}})\nonumber\\&=\mathbb{P}_g(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}}),
\end{align}
where $s_{\text{cur}} = s_{\text{after}}^k$. In words the probability of reaching a DRA state in $\ccalQ_{\text{goal}}(q_{\text{cur}})$ within the next $k^*$ iterations is equal to the probability of reaching one of the MDP states in $\ccalX_{\text{goal}}(q_{\text{cur}})$ that are $k^*$ hops (i.e., MDP transitions) away from $x_{\text{cur}}$. Observe that there are different superscripts in $q_{\text{after}}^{k+k^*+1}$ and $x_{\text{after}}^{k+k^*}$. As discussed earlier, the reason is that, by definition of the DRA transition rule, once the state $x_{\text{after}}^{k+k^*}$ is reached at iteration $k+k^*$, then at the next iteration $k+k^*+1$, the DRA state in $\ccalQ_{\text{goal}}(q_{\text{cur}})$ will be reached.

Thus, to show \eqref{eq:compSample3}, it suffices to show that
\begin{align}\label{eq:toshow}
   &\mathbb{P}_b(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}})>\nonumber\\&\mathbb{P}_g(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}}), 
\end{align}
where $s_{\text{cur}} = s_{\text{after}}^k$.
%$\mathbb{P}_b(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}})>\mathbb{P}_g(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}})$, where $s_{\text{cur}} = s_{\text{after}}^k$.
%, it suffices to show that the probability of reaching a state $x$ that belongs to $\ccalX_{\text{goal}}(q_{\text{cur}}=q_{\text{after}^k})$ after $k^*=J_{x_{\text{cur}},\ccalX_{\text{goal}}}$ iterations is greater when bias is introduced in the exploration phase.
%
By construction of the set $\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})$, we have that 
\begin{align}\label{eq1}
    &\mathbb{P}_b(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}}=s_{\text{after}}^{k})=\nonumber\\&\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}})
\end{align}
and, similarly, that 
\begin{align}\label{eq2}
    &\mathbb{P}_g(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}}=s_{\text{after}}^{k})=\nonumber\\&\prod_{m=1}^{k^*} \mathbb{P}_g(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}}),
\end{align}
where the current PMDP state on the right hand side in \eqref{eq1}-\eqref{eq2} is $s_{\text{cur}} = s_{\text{after}}^{k+m-1}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-2})$.
%$\mathbb{P}_b(x_{\text{after}}^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}})=\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^k)$
%$ \mathbb{P}_b(q_{\text{after}}^{k+k^*+1}\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}} = s_{\text{after}}^k)=\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^k)$; the same also holds for the $\epsilon$-greedy policy.
Thus, to show \eqref{eq:toshow}, it suffices to show the following inequality:
\begin{align}\label{eq:toshow2}
    &\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}})>\nonumber\\ & \prod_{m=1}^{k^*}\mathbb{P}_g(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}}).
\end{align}
where $s_{\text{cur}} = s_{\text{after}}^{k+m-1}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-2})$.

%Due to Proposition \ref{prop:sampleEf1}, we have that at the next iteration $k+1$, it holds that
By assumption, \eqref{eq:AsAvP} holds for all subsequent iterations $[k,k+k^*]$ and for all  $x\in\ccalX_{\text{closer}}(x_{\text{cur}})$, and, therefore, by applying Proposition \ref{prop:sampleEf1} to any iteration $k+m$, $m\in [1,k^*]$, we have that 
\begin{align}\label{eq:compSampleThm}
    &\mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})>\nonumber\\ & \mathbb{P}_g(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})
\end{align}
for all $m\in [1,k^*]$ and $s_{\text{cur}} = s_{\text{after}}^{k+m-1}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-2})$. Multiplying the inequalities \eqref{eq:compSampleThm} for all $m\in [1,k^*]$ yields \eqref{eq:toshow2} completing the proof.
%By definition of $k^*$ and the set $\ccalX_{\text{closer}}$, we have that $\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^k)$ is the probability that starting from $x_{\text{after}}^k$,
%\end{proof}


==> files/proofs2.tex <==
To prove Theorem \ref{thm:sampleEf2}
\begin{prop}\label{prop:sampleEf2}%[Comparative Sample Efficiency]
If the biased action $a_b$ is selected as per \eqref{eq:a_b} biasing exploration towards $x_b$, then then it holds that 
\begin{equation}\label{eq:compSample2}
    \mathbb{P}_b(x_{\text{after}}=x_b)> \mathbb{P}_g(x_{\text{after}}=x_b),
\end{equation}
where $\mathbb{P}_g(x_{\text{after}}=x_b)$ and $\mathbb{P}_b(x_{\text{after}}=x_b)$ denote the probability of reaching at the next iteration of the current RL episode the state $x_b$ starting from $x_{\text{cur}}$ without and with bias introduced in the exploration phase, respectively.
\end{prop}

\begin{proof}
The probability of reaching a state $s_{\text{after}}$ where $x_{\text{after}}=x_b$ under a policy $\mu(s)$ is: $$\sum_{a\in\ccalA(x_{\text{cur}})}\mu(s_{\text{cur}},a)P(x_{\text{cur}},a,x_b).$$ Thus, we have that:
\begin{align}\label{eq:diffCor1}
    &\mathbb{P}_b(x_{\text{after}}=x_b)- \mathbb{P}_g(x_{\text{after}}=x_b)=\nonumber\\&\sum_{a\in\ccalA(x_{\text{cur}})}P(x_{\text{cur}},a,x_b)(\mu_b(s_{\text{cur}},a)-\mu_\epsilon(s_{\text{cur}},a)).
\end{align}

Following exactly the same steps as in the proof of Proposition \ref{prop:sampleEf1}, we get that $\mathbb{P}_b(x_{\text{after}}=x_b)- \mathbb{P}_g(x_{\text{after}}=x_b)>0$ if     $P(x_{\text{cur}},a_b,x_b)>\sum_{a\in\ccalA(x_{\text{cur}})}\frac{P(x_{\text{cur}},a,x_b)}{|\ccalA(x_{\text{cur}})|}$ which trivially holds due to \eqref{eq:a_b}. Specifically, given $x_{\text{cur}}$ and $x_b$, we have that $P(x_{\text{cur}},a,x_b)\geq P(x_{\text{cur}},a,x_b)$ for all $a\in\ccalA(x_{\text{cur}})$. Thus, $P(x_{\text{cur}},a,x_b)$ must be greater than $\sum_{a\in\ccalA(x_{\text{cur}})}\frac{P(x_{\text{cur}},a,x_b)}{|\ccalA(x_{\text{cur}})|}$, i.e., the average transition probability over the actions $a$ completing the proof.
%
\end{proof}

%Observe that the result in Corollary \ref{thm:sampleEf2} is weaker than then one presented in Proposition \eqref{prop:sampleEf1}. In fact, Proposition \eqref{prop:sampleEf1} shows that if \eqref{eq:AsAvP} holds, then the probability of reaching \textit{any} state in $\ccalX_{\text{closer}}$ is greater when bias is introduced in the $\epsilon$ greedy policy. To the contrary, Corollary \ref{thm:sampleEf2} shows if \eqref{eq:AsAvP} does not hold for all $ x\in\ccalX_{\text{closer}}$, then the probability of reaching \textit{the state} $x_b\in\ccalX_{\text{closer}}$ is greater when bias is introduced in the $\epsilon$ greedy policy.

\subsection{Main Proof}

%\begin{proof}
To show this result, we follow a similar analysis as in the proof of Theorem \ref{thm:sampleEf}. Let $a_b^k$ and $x_b^k$ be the biased action and the state towards which $a_b^k$ is biased to, respectively, at iteration $k$. To show this result, we will show that the probability of reaching a state $x_r$ within the next $k^*$ iterations that satisfies $\delta_D(q_\text{cur},L(x_r))\in\ccalQ_{\text{goal}}(q_{\text{cur}})$ while avoiding all other MDP states that can enable a transition from $q_{\text{cur}}=q_{\text{after}}^{k}$ to any other DRA state is higher when bias is introduced in the exploration phase. In what follows, we show that this property holds for $x_r=x_{b}^{k+k^*}$. 
%\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})


In math, it suffices to show that
\begin{align}\label{eq:toshowCor1}
   &\mathbb{P}_b(x_{\text{after}}^{k+k^*}=x_b^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}})>\nonumber\\&\mathbb{P}_g(x_{\text{after}}^{k+k^*}=x_b^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})~|~s_{\text{cur}}), 
\end{align}
where $s_{\text{cur}} = s_{\text{after}}^k$. If fact, if $x_{\text{after}}^{k+k^*}=x_b^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})$ is true, then this means that (i) for all iterations $k+m$, $m\in[1,k^*]$ we have that $q_{\text{after}}^{k+m}=q_{\text{after}}^k$ by construction of the sets $\ccalX_{\text{closer}}$ (see Remark \ref{rem:shortestPath}) and that (ii) iteration $k+k^*+1$ transition from $q_{\text{after}}^{k+k^*}$ to a DRA state $q_{\text{after}}^{k+m}\in\ccalQ_{\text{goal}}(q_{\text{cur}})$ will be enabled since $x_{\text{after}}^{k+k^*}=x_b^{k+k^*}\in\ccalX_{\text{closer}}^{k^*}(x_{\text{cur}})$ and by definition of the set $\ccalX_{\text{closer}}^{k^*}\subseteq\ccalX_{\text{goal}}^{x_{\text{after}}^k}$.

To show \eqref{eq:toshowCor1}, recall that the biased action $a_b^{k+m}$ satisfies $a_b^{k+m} = \argmax_{a\in \ccalA(x_{\text{cur}})} P(x_{\text{cur}},a,x_b^{k+m})$ for all  subsequent iterations  $k+m$, $m\in [0,k^*]$.
%First, recall by definition of the state $x_b^{k+m}$, we have that $x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{cur}})$, where $x_{\text{cur}}=x_{\text{after}}^{k+m-1}$.
%construction of the sets $\ccalX_{\text{closer}}^{k+m}$
%By assumption, the biased action $a_b^{k+m}$ satisfies $a_b^{k+m} = \argmax_{a\in \ccalA(x_{\text{cur}})} P(x_{\text{cur}},a,x_b^{k+m})$ for all  subsequent iterations  $k+m$, $m\in [0,k^*]$.
Then, %assuming that at any iteration $k+m-1$, the current product MDP state is $s_{\text{cur}}=s_{\text{after}}^{k+m-1}=(x_b^{k+m-1}, q_{\text{cur}}^k)$
%$s_{\text{cur}} = s_{\text{after}}^{k+m-1}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-2})$
by applying Corollary \ref{thm:sampleEf2}, we have that

\begin{align}\label{eq:abPcor}
    &\mathbb{P}_g(x_{\text{after}}^{k+m}=x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})|s_{\text{cur}})>\nonumber\\& \mathbb{P}_b(x_{\text{after}}^{k+m}=x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})|s_{\text{cur}}),
\end{align}
for all $m\in[1,k^*]$. The state $s_{\text{cur}}$ in \eqref{eq:abPcor} is defined as  $s_{\text{after}}^{k+m-1}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-2})$, for all $m\in[1,k^*]$.
%
Multiplying the inequalities \eqref{eq:abPcor} for all $m\in[1,k^*]$ yields
\begin{align}\label{eq:abP1cor}
       &\boldsymbol\mu_{m=1}^{k^*}\mathbb{P}_g(x_{\text{after}}^{k+m}=x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})|s_{\text{cur}})>\nonumber\\& \boldsymbol\mu_{m=1}^{k^*}\mathbb{P}_b(x_{\text{after}}^{k+m}=x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})|s_{\text{cur}}),
\end{align}
which is equivalent to \eqref{eq:toshowCor1} by construction of the set $\ccalX_{\text{closer}}^{k^*}(x_{\text{after}}^k)$, as in the proof of Theorem \ref{thm:sampleEf}, completing the proof.
%which means that the probability of following the path, i.e., the sequence of MDP states $x_b^{k+1},x_b^{k+2},\dots,x_b^{k+k^*}$ is higher when bias is introduced in the exploration phase. 
%Then we have that:
%\begin{align}\label{eq:compSampleCor}
%    &\mathbb{P}_b(x_{\text{after}}^{k+m}=x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})>\nonumber\\ & \mathbb{P}_g(x_{\text{after}}^{k+m}=x_b^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})
%\end{align}

%it suffices to show that the probability of reaching a state $x$ that belongs to $\ccalX_{\text{goal}}(q_{\text{cur}}=q_{\text{after}^k})$ after $k^*=J_{x_{\text{cur}},\ccalX_{\text{goal}}}$ iterations is greater when bias is introduced in the exploration phase. By definition of the set $\ccalX_{\text{closer}}$, we have that $ \mathbb{P}_b(q_{\text{after}}^{k+k^*+1}\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}} = s_{\text{after}}^k)=\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^k)$; the same also holds for the $\epsilon$-greedy policy. Thus, to show \eqref{eq:compSample3}, it suffices to show the following inequality:
%\begin{align}\label{eq:show}
%    &\prod_{m=1}^{k^*} \mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})>\nonumber\\ & \prod_{m=1}^{k^*}\mathbb{P}_g(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1}).
%\end{align}

%Due to Proposition \ref{prop:sampleEf1}, we have that at the next iteration $k+1$, it holds that
%Since by assumption, \eqref{eq:AsAvP} holds for the all subsequent iterations $[k,k+k^*]$ and for all  $x\in\ccalX_{\text{closer}}(x_{\text{cur}})$, then by applying Proposition \ref{prop:sampleEf1} to any iteration $k+m$, $m\in [1,k^*]$, we have that 
%\begin{align}\label{eq:compSampleThm}
%    &\mathbb{P}_b(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})>\nonumber\\ & \mathbb{P}_g(x_{\text{after}}^{k+m}\in\ccalX_{\text{closer}}(x_{\text{after}}^{k+m-1})~|~s_{\text{cur}} = s_{\text{after}}^{k+m-1})
%\end{align}
%for all $m\in [1,k^*]$. Multiplying the inequalities \eqref{eq:compSampleThm} for all $m\in [1,k^*]$ yields \eqref{eq:show} completing the proof.
%\end{proof}


==> files/theory.tex <==
%\red{[needs to be polished a lot....]}

%\begin{prop}[Correctness]
%If Algorithm \ref{alg:RRT} terminates successfully, then the resulting path $\bbp_{0:H}$ satisfies the LTL property $\phi$.
%\end{prop}
%\begin{proof}
%This result is true by construction of Algorithm \ref{alg:RRT}. Specifically, while the robots navigate in the workspace to reach the target DFA state $q_D^{\text{target}}$ from the current DFA state $q_D(t)$, they always check if the next observation $L(\bbp(t+1))$ violates the LTL formula $\phi$. If this is not the case, for all $t\geq 0$, the robots will eventually reach all subsequent target DFA states. Since the target DFA states are selected so that they are always one hop closer to the final state $q_F^{\text{feas}}$ than $q_D(t)$ is (see \eqref{eq:targetDFA}), this means that eventually the robots will reach $q_F^{\text{feas}}$ and, therefore, they will satisfy $\phi$ completing the proof.
%\end{proof}

%(ii) there do not exist regions $r_i$ and $r_e$, such that $r_i\subseteq r_e$ and 
%and (ii) there do not exist regions $r_i$ that are accessible only after visiting first
In this section, we show that any $(\epsilon,\delta)-$greedy policy achieves policy improvement; see Proposition \ref{prop:polImprov}. Also, we show that the proposed biased exploration strategy results in learning control policies faster than policies that rely on uniform-based exploration. Specifically, we show that during an RL episode the probability of reaching DRA states that are closer to the accepting states is higher when bias is introduced in the exploration phase. The latter is formally shown in Theorems \ref{thm:sampleEf} and \ref{thm:sampleEf2}. 

In the following proposition, we show that policy improvement is guaranteed for any $(\epsilon,\delta)-$greedy policy.
\begin{prop}[Policy Improvement]\label{prop:polImprov}
For any $(\epsilon,\delta)$-greedy policy $\boldsymbol{\mu}$, the updated $(\epsilon,\delta)$-greedy policy $\boldsymbol{\mu}$ obtained after updating the state-action value function $Q^{\boldsymbol{\mu}}(s,a)$ satisfies $U^{\boldsymbol{\mu'}}(s)\geq U^{\boldsymbol{\mu}}(s)$, for all $s\in\ccalS$.%\footnote{} 
$\hfill\Box$
\end{prop}

\begin{proof}
To show this result, we follow the same steps as in the policy improvement result for the $\epsilon$-greedy policy \cite{rlbook}. For simplicity of notation, hereafter we use $m=|\ccalA_{\mathfrak{P}}(s)|$. Thus, we have that:
\begin{align}
    &U^{\boldsymbol\mu'}(s)=\sum_{a\in\ccalA_{\mathfrak{P}}(s)}\boldsymbol\mu'(s,a)Q^{\boldsymbol\mu}(s,a)\\
    &=\frac{\delta_{e}}{m}\sum Q^{\boldsymbol\mu}(s,a)+(1-\epsilon)\max_{a\in\ccalA_{\mathfrak{P}}(s)}Q^{\boldsymbol\mu}(s,a)\\&+\delta_b Q^{\boldsymbol\mu}(s,a_b)\\
    &\geq\frac{\delta_{e}}{m}\sum Q^{\boldsymbol\mu}(s,a)\nonumber\\&+(1-\epsilon)\sum_{a\in\ccalA_{\mathfrak{P}}(s)}\left(\frac{\boldsymbol\mu(s,a)-\frac{\delta_e}{m}-\mathbb{I}_{a=a_b}\delta_b}{1-\epsilon}\right)Q^{\boldsymbol\mu}(s,a)\label{eq:sum1}\\&+\delta_b Q^{\boldsymbol\mu}(s,a_b)
    =\sum_{a\in\ccalA_{\mathfrak{P}}(s)}\boldsymbol\mu(s,a)Q^{\boldsymbol\mu}(s,a)=U^{\boldsymbol\mu}(s)
\end{align}
where the inequality holds because the summation in \eqref{eq:sum1} is a weighted average with non-negative weights  summing to $1$, and as such it must be less than the largest number averaged.
%\begin{align}
%    &Q(\bbx,\boldsymbol{\mu}'(\bbx))=\sum_{\bba\in\ccalA}\boldsymbol{\mu}'(\bba|\bbx)Q(\bbx,\boldsymbol{\mu}(\bbx))=\nonumber\\
%\end{align}
\end{proof}

In Proposition \ref{prop:polImprov}, the equality $U^{\boldsymbol{\mu'}}(s)= U^{\boldsymbol{\mu}}(s)$, for all $s\in\ccalS$, holds if $\boldsymbol\mu=\boldsymbol\mu'=\boldsymbol\mu^*$, where $\boldsymbol\mu^*$ is the optimal policy \cite{rlbook}.
%\textcolor{red}{read the book and mention that this implies convergence to optimal action value}
%Let $s_{\text{cur}}=[x_{\text{cur}},q_{\text{cur}}]$ be the current product state during an RL episode. Also, let $\ccalX_{\text{next}}(s_{\text{cur}})\subseteq\ccalX$ be a set of MDP states that if the robot eventually reaches, then transition to a product state $s_{\text{next}}=[x_{\text{next}},q_{\text{next}}$ will occur, where $x_{\text{next}}\in\ccalX_{\text{next}}$ and $q_{\text{next}}\in\ccalQ_{\text{next}}$ (see \eqref{eq:Qnext}). Formally, $\ccalX_{\text{next}}(s)$ is defined as follows:
%
%\begin{equation}
%\ccalX_{\text{next}}(s) = \{x\in\ccalX~|~\delta_D(q,L(x))=q_{\text{next}}\in\ccalQ_{\text{next}}\}
%\end{equation}
%
%Next, for each $x_{\text{next}}\in\ccalX_{\text{next}}(s)$, we compute all MDP states, denoted $\ccalX_{\text{closer}}(s)\subseteq\ccalX_{\text{next}}$ that are one hop reachable from $x_{\text{cur}}$ and they are closer to $\ccalX_{\text{next}}(s)$ than $x_{\text{cur}}$ is, as per \eqref{eq:distM}. To this end, we compute the shortest path from $x_{\text{cur}}$ to $x_{\text{next}}$, for all $x_{\text{next}}\in\ccalX_{\text{next}}(s)$, denoted by $p^k=p_0^k,p_1^k,\dots,p_{H_k}^k$, where the index $k$ refers to the $k$-th state in $\ccalX_{\text{next}}$, $p_0^k=x_{\text{cur}}$, and $p_{H_k}^k=x_{\text{next}}$. We collect all states $p_1^k$ in a set denoted by  $\ccalX_{\text{closer}}(s)\subseteq\ccalX$.
%
%To this end, we define first the `distance' of an MDP state $x_{\text{cur}}$  from the set $\ccalX_{\text{next}}(s)$ as:
%
%\begin{equation}
%    ..
%\end{equation}
%are per $d_{\mathfrak{M}}$.
%
In Theorem \ref{thm:sampleEf}, we formally show the effect of introducing bias in the exploration phase; its proof can be found in Appendix \ref{sec:proof1}. Specifically, we show that the proposed biased exploration strategy results in increasing the probability of reaching DRA states that are closer to the accepting states within a finite number of iterations.
%In what follows, we compare the sample-efficiency of the proposed control policy against the $\epsilon$-greedy policy. 
Specifically, we consider the $(\epsilon,\delta)$-greedy policy defined in \eqref{eq:policy0} and the $\epsilon$-greedy policy that considers random/uniform exploration. As per the $\epsilon$-greedy policy, the greedy action is selected with probability $1-\epsilon$ and a random action is selected with probability $\epsilon$. To make this comparative analysis meaningful, hereafter, we assume that probability of exploration $\epsilon=\delta_b+\delta_e$ is the same for both policies; this probability of selecting the greedy action is the same, as well. Note that the $\epsilon$-greedy policy can be recovered by removing bias from the $(\epsilon,\delta)$-greedy policy, i.e., by setting $\delta_b=0$. 
%Also, let $s_{\text{cur}}=(x_{\text{cur}},q_{\text{cur}})$ be current product MDP state during an RL episode of Algorithm \ref{alg:RL-LTL}. Then, we show that during the current RL episode, the probability of making progress towards accomplishing the LTL task is higher when the biased greedy policy is employed. This result is formally stated in Theorem \ref{thm:sampleEf}. 




%Next, we show that the probability
\begin{theorem}[Effect of Bias]\label{thm:sampleEf}
%Let $s_{\text{after}}^k=(x_{\text{after}}^k,q_{\text{after}}^k)$ denote the product MDP state that will be reached after $k$ iterations (\texttt{iterations} in Algorithm \ref{alg:RL-LTL}) during an RL episode starting from $s_{\text{cur}}$. %, i.e.,  $s_{\text{after}}^0=s_{\text{cur}}$. 
%Let $s_{\text{after}}^k$ denote be the current product state of the robot during an RL episode, i.e., $s_{\text{cur}} = s_{\text{after}}^k$. 
Let $s_{\text{after}}^k=(x_{\text{after}}^k,q_{\text{after}}^k)$ be the product state that is reached at the $k$- iteration (denoted by \texttt{iterations} in Algorithm \ref{alg:RL-LTL}) of the current RL episode. Also, let $s_{\text{cur}} = s_{\text{after}}^k$. If the following condition
\begin{equation}\label{eq:AsAvP}
    P(x_{\text{cur}},a_b,x_b)>\sum_{a\in\ccalA(x_{\text{cur}})}\frac{P(x_{\text{cur}},a,x)}{|\ccalA(x_{\text{cur}})|}, \forall x\in\ccalX_{\text{closer}}(x_{\text{cur}}),
\end{equation}
%\eqref{eq:AsAvP} holds for all $x\in\ccalX_{\text{closer}}(x_{\text{cur}})$ and 
holds for all subsequent $k^*=J_{x_{\text{cur}},\ccalX_{\text{goal}}}$  iterations, then the probability of reaching a DRA state in $\ccalQ_{\text{goal}}(q_{\text{cur}})$ (see \eqref{eq:Qnext}) is higher when bias is employed, i.e., 
\begin{align}\label{eq:compSample3}
    &\mathbb{P}_b(q_{\text{after}}^{k+k^*+1}\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}} = s_{\text{after}}^k)>\nonumber\\&  \mathbb{P}_g(q_{\text{after}}^{k+k^*+1}\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}} = s_{\text{after}}^k), 
\end{align}
where (i) $\mathbb{P}_g(\cdot)$, and $\mathbb{P}_b(\cdot)$ denote the probability of reaching a state that belongs to $\ccalQ_{\text{goal}}(q_{\text{cur}})$ after $k^*$ iterations starting from $s_{\text{cur}}$ without and with bias in the exploration phase, respectively, and (ii) $k^*$ is the minimum number of iterations required to reach $\ccalQ_{\text{goal}}(q_{\text{cur}})$ starting from $q_\text{cur}$ by definition of the cost $J_{x,x'}$.$\hfill\Box$
\end{theorem}



%Note that \eqref{eq:AsAvP} may not hold for all iterations within an RL episode because of the MDP structure. Also, 

%%
%By construction of the biased policy, if a biased action that satisfies \eqref{eq:AsAvP0} does not exist, then it selected as per \eqref{eq:a_b}, i.e., $ a_b = \argmax_{a\in \ccalA(x_{\text{cur}})} \hat{P}(x_{\text{cur}},a,x_b)$.
%may not hold because of the currently learned MDP structure. In this case, the biased action is selected as per \eqref{eq:a_b}. 
%In what follows, we show that if the biased action is selected as per \eqref{eq:a_b} and it satisfies 
%%

Theorem \ref{thm:sampleEf2} shows the effect of bias in case a biased action cannot be selected as per \eqref{eq:AsAvP0}.
%By construction of the biased policy, if a biased action $a_b$ that satisfies \eqref{eq:AsAvP0} does not exist, then it selected as per \eqref{eq:a_b}, i.e., $ a_b = \argmax_{a\in \ccalA(x_{\text{cur}})} \hat{P}(x_{\text{cur}},a,x_b)$.
%%may not hold because of the currently learned MDP structure. In this case, the biased action is selected as per \eqref{eq:a_b}. 
%In Theorem \ref{thm:sampleEf2}, we show that if the biased action satisfies 
%\begin{equation}\label{eq:cond2}
%  a_b = \argmax_{a\in \ccalA(x_{\text{cur}})} P(x_{\text{cur}},a,x_b),  
%\end{equation}
%then the probability of reaching \textit{a DRA state} (and not all DRA states as in Theorem \ref{thm:sampleEf}) that is closer to the DRA accepting states is higher when bias is introduced in the exploration phase. Notice that (i) \eqref{eq:cond2} considers the actual probabilities and not the estimated ones as in \eqref{eq:a_b} and (ii) that \eqref{eq:cond2} is a more relaxed condition than \eqref{eq:AsAvP0} is.
%and that \eqref{eq:cond2} is weaker result than Theorem \ref{thm:sampleEf}. In fact, Theorem \ref{thm:sampleEf} shows that if the biased action  satisfies \eqref{eq:AsAvP} (which is a stronger requirement than \eqref{eq:cond2}) then the probability of reaching \textit{all DRA states} that are closer to the DRA accepting states and can be reached within $k^*$ iterations is higher when bias is introduced in the exploration phase. %To formally state and show this result, we need first to state the following corollary.

%of making progress towards accomplishing the assigned LTL formula (i.e., reaching a subset of of DRA states that are closer to the DRA accepting states than the current DRA state) within the minimum number of iterations (denoted by $k^*$ in Theorem \ref{thm:sampleEf}) required

%that if the biased action is always selected as per \eqref{eq:a_b}, then probability of making progress towards satisfying the LTL formula by following a specific path of length $k^*$ is greater when bias is introduced in the exploration phase. Recall from Theorem \ref{thm:sampleEf} that $k^*$ is the the minimum number of iterations required to make progress towards accomplishing the LTL task (i.e., getting closer to the accepting DRA states).  



\begin{theorem}[Effect of Bias on Sample Efficiency]\label{thm:sampleEf2}
%Let $s_{\text{after}}^k=(x_{\text{after}}^k,q_{\text{after}}^k)$ denote the product MDP state that will be reached after $k$ iterations (\texttt{iterations} in Algorithm \ref{alg:RL-LTL}) during an RL episode starting from $s_{\text{cur}}$. %, i.e.,  $s_{\text{after}}^0=s_{\text{cur}}$. 
Let $s_{\text{after}}^k=(x_{\text{after}}^k,q_{\text{after}}^k)$ be the product state reached at the $k$- iteration (denoted by \texttt{iterations} in Algorithm \ref{alg:RL-LTL}) of the current RL episode. Also, let $s_{\text{cur}} = s_{\text{after}}^k$, for some $k\geq 0$. If the biased action $a_b$ satisfies
\begin{equation}\label{eq:cond2}
  a_b = \argmax_{a\in \ccalA(x_{\text{cur}})} P(x_{\text{cur}},a,x_b),  
\end{equation}%\eqref{eq:cond2} %$a_b = \argmax_{a\in \ccalA(x_{\text{cur}})} P(x_{\text{cur}},a,x_b)$ (see also \eqref{eq:a_b}), 
for all subsequent $k^*=J_{x_{\text{cur}},\ccalX_{\text{goal}}}$ iterations, then we have that there exists a DRA state $q_b\in \ccalQ_{\text{goal}}(q_{\text{cur}})$ such that
\begin{align}\label{eq:compSample3}
    &\mathbb{P}_b(q_{\text{after}}^{k+k^*+1}=q_b\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}} = s_{\text{after}}^k)>\nonumber\\&  \mathbb{P}_g(q_{\text{after}}^{k+k^*+1}=q_b\in\ccalQ_{\text{goal}}(q_{\text{cur}})~|~s_{\text{cur}} = s_{\text{after}}^k), 
\end{align}
where $\mathbb{P}_b$ and $\mathbb{P}_g$ are defined as in Theorem \ref{thm:sampleEf}. $\hfill\Box$%$k^*$ is the minimum number of iterations required to reach $\ccalQ_{\text{goal}}(q_{\text{cur}})$ starting from $q_\text{cur}$ by definition of the cost $J_{x,x'}$ and $\ccalQ_{\text{goal}}(q_{\text{cur}})$ is defined in \eqref{eq:Qnext}.
\end{theorem}


\begin{rem}[Selecting exploration parameters $\delta_b$ and $\delta_e$]\label{rem:deltas}
Observe in Algorithm \ref{alg:RL-LTL} that the biased action is selected so that it satisfies \eqref{eq:AsAvP0} and not \eqref{eq:AsAvP}, since the actual transition probabilities are a priori unknown. Similarly, in case \eqref{eq:AsAvP0} cannot be satisfied, the biased action is selected as per \eqref{eq:a_b} and, therefore, it may not satisfy \eqref{eq:cond2}. The only difference between \eqref{eq:AsAvP0} and \eqref{eq:AsAvP} and between \eqref{eq:a_b} and \eqref{eq:cond2} is that \eqref{eq:AsAvP0} and \eqref{eq:a_b} employ the currently estimated transition probabilities while \eqref{eq:AsAvP} and \eqref{eq:cond2} consider the actual, but unknown, transition probabilities. As a result, the selected biased action $a_b$ may not satisfy \eqref{eq:AsAvP} even if it satisfies \eqref{eq:AsAvP0} due to inaccurate estimated transition probabilities; the same holds for \eqref{eq:a_b} and \eqref{eq:cond2}. Thus, to enjoy the fast convergence properties implied by Theorems \ref{thm:sampleEf} and \ref{thm:sampleEf2}, initially, we select $\delta_e>\delta_b$ while $\delta_e$ converges to $0$ faster than $\delta_b$. Intuitively, this allows to initially perform random exploration to learn an accurate enough MDP model which is then exploited to bias exploration towards directions that will drive the system closer to the DRA accepting states. Finally, observe that \eqref{eq:cond2} is a more relaxed condition than \eqref{eq:AsAvP}. %Note that selection of a biased action that satisfies \eqref{eq:AsAvP} or \eqref{eq:cond2} does not require perfect knowledge knowledge
\end{rem}




%\begin{rem}
%Note that assumption \eqref{eq:AsAvP} may not hold for arbitrary MDP structures. In words, \eqref{eq:AsAvP} requires, at every iteration of each RL episode of Algorithm \ref{alg:RL-LTL}, given the action $a_b$ and the MDP state $x_b$, the transition probability $P(x_{\text{cur}},a_b,x_b)$ to be greater than the average transition probability from the current state $x_{\text{cur}}$ to a state $x\in\ccalX_{\text{closer}}$ over the action space $\ccalA(x_\text{cur})$, for all $x\in\ccalX_{\text{closer}}(x_{\text{cur}})$. In Section \ref{sec:Sim}, we show that even \eqref{eq:AsAvP} does not hold, Algorithm \ref{alg:RL-LTL} is more sample-efficient due to the bias introduced in the exploration phase.
%\end{rem}








